HufuNet: Embedding the Left Piece as Watermark and Keeping the Right Piece for Ownership Verification in Deep Neural Networks

Due to the wide use of highly-valuable and large-scale deep neural networks (DNNs), it becomes crucial to protect the intellectual property of DNNs so that the ownership of disputed or stolen DNNs can be verified. Most existing solutions embed backdoors in DNN model training such that DNN ownership can be verified by triggering distinguishable model behaviors with a set of secret inputs. However, such solutions are vulnerable to model fine-tuning and pruning. They also suffer from fraudulent ownership claim as attackers can discover adversarial samples and use them as secret inputs to trigger distinguishable behaviors from stolen models. To address these problems, we propose a novel DNN watermarking solution, named HufuNet, for protecting the ownership of DNN models. We evaluate HufuNet rigorously on four benchmark datasets with five popular DNN models, including convolutional neural network (CNN) and recurrent neural network (RNN). The experiments demonstrate HufuNet is highly robust against model fine-tuning/pruning, kernels cutoff/supplement, functionality-equivalent attack, and fraudulent ownership claims, thus highly promising to protect large-scale DNN models in the real-world.

==> arxiv2021 HufuNet/overview.tex <==
\section{Motivation}
\label{sec:Motivation}


\begin{figure}[t]
\centering
\epsfig{figure=fig/motivation.png, width=0.5\textwidth} 
\caption{\textbf{Motivation Example}}
\label{fig:motivation}
\end{figure}






\subsection{Threat Example}
\shengzhi{Motivation examples means you tell a story: a) A model owner releases their model (complicated and accurate) on github, b) adversary identifies its value and clones it, c. To avoid legal issues, adversary fine-tunes (XXX approaches) the model and adds his own watermark, d) Adversary commercializes it (make it black box as well) and gets revenue. Then you want to use the story to emphasize the need of our approach: a) black box model from adversary, so we need to probe. But since the model is complicated and adversary has done pruning, the results of probing may not be convincing. Therefore, white box verification is needed.}

As the advance of AI techniques, neural networks are involving in various complicated tasks, e.g., autonomous driving, speech recognition, remote diagnosis, etc. Such tasks usually rely on DNN models trained on a large amount of data using intensive GPU resources.
For instance, AlexNet paper[] it’s stated that “our network takes between five and six days to train on two GTX 580 3GB GPUs”. \shengzhi{Give an example of a real world complicated model trained using XXX data and XXX GPU for XXX days.} Hence, the IP of DNN models has become a vital topic in the AI community. 

Consider an example as shown in Figure\ref{fig:motivation}, Alice makes great efforts to design a complicated and accurate neural network $DNN_{Alice}$ that performs well on the main task, and embed a backdoor[] watermark to $DNN_{Alice}$. Then he publishes $DNN_{Alice}$ to models sharing platform, such as GitHub and Google Cloud AI platform []. After that, an attacker Bob thinks that $DNN_{Alice}$ is very valuable, and then stealing it. To avoid legal issues, Bob fine-tunes, prunes the model and adds his own backdoor[] watermark, generating $DNN_{Bob}$. Next, Adversary commercializes it in black box and gets revenue.  

In view of this situation, Alice needs to claim ownership of the stolen model $DNN_{Bob}$. Alice first performs black box verification on $DNN_{Bob}$, but at this time, Bob can also have some key samples constructed by AEs or from his new constructed backdoor for fraudulent claims of ownership. Moreover since the model is complicated and adversary has done pruning, the results of probing by backdoor may not be convincing. 

%\begin{figure}[t]
%\centering
%\epsfig{figure=fig/table_attacker.png, width=0.5\textwidth} 
%\caption{\textbf{Capability of Attacker}}
%\label{fig:table_attacker}
%\end{figure}

\begin{table}
\centering
\footnotesize
\caption{Capability of Watermark}
\label{tab:Capability of Attacker}
\begin{tabular}{m{2.5cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1.4cm}
<{\centering}}
\hline
\textbf{ }& \textbf{Elementary level}& \textbf{Intermediate level}& \textbf{Advanced level}\\
\hline \hline
\textbf{Fraudulent claims of ownership} & \text{\Checkmark}& \text{\Checkmark}& \text{\Checkmark}\\ \hline
\textbf{Access to White Box}& \text{-} &\text{\Checkmark}& \text{\Checkmark} \\ \hline
\textbf{Pruning and Fine-tuning}& \text{-} &\text{-}& \text{\Checkmark} \\ \hline
\textbf{Watermark Rewrite}& \text{-} &\text{-}& \text{\Checkmark} \\ \hline
\end{tabular}
\end{table}

\shengzhi{The Table needs revision. It should show how existing works and ours perform on those metrics listed in the first column.}

Moreover, we classify several levels of attackers according to the capability our attacker can have as show in Figure \ref{fig:table_attacker}.
These attackers cause great challenges to current backdoor watermarking methods. Therefore, some watermark that can play an arbitration role in ownership verification is needed, we propose $HufuNet$ which can give an arbitration result of ownership in white box. Only in this way, can Alice verify the ownership of $DNN_{Bob}$ without any controversy.


\begin{comment}
A well-trained DNN is a valuable intellectual property (IP) for its owners, officials hope to use legal measures to protect the intellectual property of model owners. And the role of the watermark is primarily to protect the IP from being infringed.

The potential security risks of the IP of DNN are watermark removing and fraudulent claims of ownership. In terms of watermark removing, previous work \textcolor{red}{[leveage] [fine-prune] [evasion]} showed that attacker $\mathbb{A}$ can increase learning rates to fine-tuning or pruning to effectively remove the black box watermark. In terms of fraudulent claims of ownership, attacker $\mathbb{A}$ can generate some AEs [X] to fraudulent claim of ownership. Both of these risks are huge challenges to black box watermark. To address the above problems, we propose a new watermark ownership framework that provides the first black box verification, and then white box ownership verification with a high robustness protection mechanism.

For the $DNN_{valid}$ of disputed ownership, we first perform a robust black box watermark verification. If the verification result is under a high degree of confidence, we will prove the ownership of $DNN_{valid}$. But in the following two cases, the black box watermarking is not enough to verify ownership, and we will utilize the more robust and trustworthy white box watermarking method. 
(1)The black box method does not prove our ownership with a high degree of confidence, but we found out it is our model through a few minor details, and then we take legal means to get the white box model of $DNN_{valid}$ for further verification. (2)Fraudulent claims of ownership. Although we can verify ownership in the black box, attackers can also generate some adversarial samples and verify them in black box. 
Similarly, we take legal means to get the white box model of $DNN_{valid}$ and performs white box verification.
\end{comment}

\begin{comment}

\subsection{Threat Model}

\shengzhi{Usually threat model is to assume the maximum capability your adversary can have. Then your approch is to deal with the worse case based on your threat model.}

The main methods of attack to eliminate the DNN watermark are pruning, fine-tuning, and watermark rewriting. Also fraudulent clams ownership attack leads to disputes over ownership. As far as these attack methods proposed, We classify several levels of attackers $\mathbb{A}$ according to the maximum capability our attacker can have as follows:

Elementary level: $\mathbb{A}$ cannot get our white box model, nor has ability of pruning, fine-tuning, watermark rewrite to our model. But he claim the ownership of our DNN rascally without any evidience.

Intermediate level:$\mathbb{A}$ does not have access to our white box model. However, they generate some AEs through queries, which in turn build trigger sets to claim ownership of the black box DNN.

Advanced level: $\mathbb{A}$ can obtain the white box model, then without pruning, fine-tuning and rewriting watermark to model. $\mathbb{A}$ didn't embed the watermark, but claimed that part of the neural network was his watermark.

Ultimate level: $\mathbb{A}$ can get access to the white box model and perform operations such as pruning and fine-tuning, further adding a similar white box secret key to claim ownership.

\end{comment}



\subsection{Design Requirements}
\shengzhi{Based on the threat model, here you can elaborate the design requirements, e.g., effectiveness, fidelity, robustness, integrity, security, etc.}

As mentioned above, we assume that attackers have a certain amount of destructive power and therefore some technical challenges need to be addressed for achieve accurate and efficient verification of watermark ownership. We conducted an in-depth analysis of the capabilities of the four levels of attackers in order to propose an excellent watermark approach.
\begin{comment}
Elementary level: Since the attacker $\mathbb{A}$ cannot get our white box model and cannot build trigger sets to verify ownership in black box, we need to design a watermark with good quality of effectiveness and integrity and security in black box verification. 

\end{comment}

Elementary level: The attacker $\mathbb{A}$ can generate some AEs to generate his trigger sample to claim ownership of our DNN, even without access to our DNN. It is a drawback to backdoor watermark to defend the attack fraudulently claim ownership. So we need to design a new watermark total different from backdoor watermark to avoid the drawback of backdoor. The new watermark shall meet the requirement as: it only can  verify the ownership of DNN which it embedded; it is difficult to fake a substitute watermark to claim ownership.

Intermediate level: Owning $\mathbb{A}$ can obtain the white box DNN and claimed that a originally part of the DNN was his watermark. In this case, we must sure our watermark with quality that watermark is undetected by attacker and it is difficult to fake a substitute watermark only by some original part of DNN and attack's local secret.


Advanced level: Due to $\mathbb{A}$ gaining the white box model, and attacking our watermark by pruning, fine-tuning, and watermark rewriting. Therefore, we need to make sure the white box watermark is of good robust to these attacks and undetected by adversary.

Moreover, a well watermark should have guaranteed a good quality that after embedding watermark, the protected DNN can not have a significant decrease in performance.

\vspace{5pt}

==> arxiv2021 HufuNet/sections/Approach.tex <==
\section{Approach}
\label{sec:Approach}
%-------------------------------------------------------------------------------
\begin{figure*}[!t]
\centering
\epsfig{figure=fig/overview.png, width=0.80\textwidth} 
\caption{Workflow of HufuNet}
\label{fig:workflow}
\end{figure*}

%\shengzhi{In Figure 2, change To-be-protected DNN to DNN-to-be-protected. Put a space after numbers 1, 2, 3. In 3. Ownership Verification, the result of combination should be the $HufuNet_{combined}$. You can move the testing dataset a little below. Delete Embedded piece of HufuNet, Secret Piece of HufuNet and Embedded piece of $HufuNet_{retrieved}$.}
Figure~\ref{fig:workflow} shows the workflow of HufuNet in three phases: watermark generation, watermark embedding, and ownership verification. During the watermark generation phase, a model owner trains a unique neural network, HufuNet, on a public training set $D_s$ and divides its parameter space into two pieces: $Embedded\ Piece\ of\ HufuNet\ (EPH)$ as watermark, and $Secret\ Piece\ of\ HufuNet\ (SPH)$ as local secret. During the watermark embedding phase, the model owner injects the watermark EPH into the parameter space of his/her DNN model (i.e., DNN-to-be-protected) for ownership protection and trains it on a large training set $D_t$ with EPH frozen to fulfill its training task (i.e., DNN-watermarked). During the ownership verification phase, the owner extracts a watermark $EPH_{retrieved}$ from a suspect DNN model, and merges it with his/her local SPH to generate a neural network model $HufuNet_{combined}$. The owner can then test $HufuNet_{combined}$ on a public testing dataset $D_{s\_TEST}$ with the same distribution as $D_s$, and verify his/her ownership if the suspect model is embedded with the watermark EPH. Following Kerckhoffs' principle, we assume the watermark embedding algorithm and the ownership verification algorithm are public. While the adversaries may forge HufuNet from the public training dataset $D_s$, they need to use the public testing dataset $D_{s\_TEST}$ and follow the public ownership verification algorithm to claim their ownership over disputed models. 
\vspace{-3pt}
\subsection{Watermark Generation}
\label{subsec: watermark_Genaration}
%If the DNN-to-be-protected is a CNN model (RNN model, respectively), 
The structure of HufuNet consists of several convolutional layers followed by a fully connected layer. The size of each convolution kernel in HufuNet is chosen to be $3*3$ in this paper; therefore, the number of parameters for each kernel is nine. After HufuNet is trained on a public data set $D_s$, all of its convolution layers are used as watermark EPH, while the fully connected layer is kept locally as secret SPH. The size of EPH is typically much smaller than the DNN model in which EPH is embedded. 
% The following discussion is superfacial and confusing at this stage; thus I delete it.
%The reason for such design is anti-forge. With just one fully connected layer stored locally, it will be hard for adversaries to forge a HufuNet by merging their own fully connected layer with some parameters chosen from the model they steal (as the convolutional layers of their forged Hufu), which still can fulfill the required classification task\footnote{In Section \ref{subsec:Watermark Embedding}, we also associate the parameter values of EPH and the corresponding embedding locations in DNN-to-be-protected to further increase the difficulty of forging.}. 
HufuNet can be considered as a mapping from its input space to its output space: $\mathbb{R}^M_{s} \rightarrow \mathbb{R}^N_{s}$ after it is trained using the dataset $D_{s}$.
%Note that $D_{s}$ should be different from, nor a subset of the main task of the DNN-to-be-protected. Otherwise, the similarity of the main task between HufuNet and the DNN-to-be-protected may introduce high similarity between their parameter spaces in terms of distribution and variance, which facilities the attackers to deduce EPH based on statistical approaches.\lpz{I don't know why "which facilities the attackers to deduce EPH based on statistical approaches."} Therefore, we train HufuNet using the training set $D_{s}$ with a different task than the that of the DNN-to-be-protected to preserve the stealthiness of the embedded watermark. 
The mapping achieves high accuracy on a testing dataset $D_{s\_TEST}$, which has the same distribution as $D_s$. Both $D_s$ and $D_{s\_TEST}$ are released to the public for training and verifying HufuNet. Note that it is beneficial to standardize $D_s$ and $D_{s\_TEST}$ so that the adversaries cannot use arbitrary datasets to forge and verify their own HufuNet (refer to evaluation results in Section~\ref{subsec:security1}).  
%Interestingly, we find that embedding the convolution layers from the well-trained HufuNet into the DNN-to-be-protected can speed up the convergence of the latter during its training, even they target at different main tasks. For example, embedding the convolutional layers of LeNet trained on MNIST into the parameter space of VGG11 to be trained on CIFAR10 can improve the accuracy of VGG11 to 69.68\% compared with 42.17\% for the first epoch training of VGG11. We speculate the reason for such performance improvement is due to quick convergence, i.e., the capability of the well-trained convolutional layers of LeNet actually ``transferred'' to the training of VGG11, since the convolutional layers are known to extract features, not so relevant to the specific tasks of each model. \shengzhi{Check if true or not.}
%\lpz{All these five DNNs have this attribute.}

%\lpz{may be here we can change our view: we think embedding a well-trained EPH can guarantee a good quality of Fidelity. We can find a famous theory to demonstrate or experiments to verify.} Embedding the convolution layers trained on a different task into another DNN can speed up its convergence. For example, embedding the convolutional layers of LeNet trained on MNIST into the parameter space of VGG11 to be trained on CIFAR10 can improve the accuracy of VGG11 to 69.68\% compared with 42.17\% for the native training of VGG11. We believe the reason for quick convergence is that the capability of the well-trained convolutional layers of LeNet actually ``transferred'' to the training of VGG11, since the convolutional layers are known to extract features, not so relevant to the specific tasks of each model. \kai{is the reason always correct? maybe you need to refer to some famous studies to prove this.} \lpz{I have try to find the famous studies, but now, I don't find. In particular, I think this theory maybe not work, owning to our EPH was embedded into DNN-to-be-protected with parameter Completely dispersed.}

\vspace{-3pt}
\subsection{Watermark Embedding}
\label{subsec:Watermark Embedding}

We focus on CNN models in explaining HufuNet watermark embedding process, where the DNN-to-be-protected includes convolutional layers. Regarding RNN models, we simply view LSTM as one convolutional layer with $N$ kernels, each with $3*3$ parameters, to embed HufuNet watermarks.

\noindent\textbf{Embedding approach.}
Watermark EPH is embedded into the convolutional layers of DNN-to-be-protected. In this process, each convolution kernel of EPH is embedded individually into DNN-to-be-protected, which is much larger than EPH. A secret key determines the embedding location of each kernel based on its parameter values and index, to ensure the stealthiness of EPH in the parameter space of DNN-to-be-protected. The secret key should be strong enough to defend against potential attacks to detect the embedded watermark. e.g., brute force searching (refer to evaluation results in Section \ref{exp_stealthiness}).

Algorithm \ref{alg:Position-injected} shows the details of our watermark embedding approach. Line 1 initializes the variables $bitmap$, which keeps track of whether each position in DNN-to-be-protected has been embedded, and DNN-watermarked $f_{wm}$. For each convolution kernel in our watermark EPH (Line 2), we first perform an XOR operation on its index $i$ and all its $k*k$ parameter ($k=3$ in our EPH), hash the result using a secret $key$, and finally do a modulo over the number of kernels in DNN-to-be-protected to compute the embedding position (Line 3). If the position has been embedded, we simply do a linear probing to find the next available position (Line 4-6). Once the position is found, we embed the convolution kernel into the corresponding position in $f_t$ (Line 7), update $bitmap$ to indicate the position has been used (Line 8), and continue the next kernel (Line 9). Finally, we output DNN-watermarked $f_{wm}$ in Line 11. Note that the kernel parameters in EPH are used in determining where EPH is embedded in $f_t$. The owner of $f_t$ needs to keep the whole HufuNet, including EPH and SPH, for ownership verification. In the process of ownership verification, the preserved EPH is used to locate where it is embedded from a suspect model, while the values in the suspect model are not used to locate the watermark since they may have been changed in the watermark embedding process and possibly by the adversaries. 

\begin{algorithm}[t]
 	\caption{Embedding Algorithm}
 	\label{alg:Position-injected}
 	\begin{algorithmic}[1]
 	\REQUIRE $f_t$: DNN-to-be-protected; $N$: number of convolution kernels in $f_t$; $Kernel$: all kernels in EPH to be embedded;
 	 $n$: number of kernels in $Kernel$; $bitmap$: a bitmap to keep track of the usage of each position in $f_t$; $key$: a secret key 
 	\ENSURE $f_{wm}$: DNN-watermarked 
 	\STATE{$bitmap = NULL$, $f_{wm} = f_t$}
	\FOR{$i$ in $(1, n)$}
        \STATE{$position=HMAC(key,XORPMV(kernel_i) \oplus i) \% N$}
		\WHILE{$bitmap_{position}$} 
		\STATE{$position = ++position \% $ N}
		\ENDWHILE
		\STATE{$f_{wm} = EMBED(kererl_i, position, f_{wm}$)}
		\STATE{$bitmap_{position} = 1$}
		\STATE{$++i$}
	\ENDFOR
    \RETURN $f_{wm}$
\end{algorithmic}
\rule[0pt]{8.4cm}{0.05em}
\begin{tablenotes}
\footnotesize
\item{$XORPMV$ is the function to $XOR$ all the parameter values of a convolution kernel. $EMBED$ is the function to embed a convolution kernel of EPH into a specific position of $f_t$. $HMAC$ is a keyed cryptographic hash function.}
\end{tablenotes}
\end{algorithm}


\noindent\textbf{Training DNN-watermarked.} 
The DNN-to-be-protected $f_t$ is a mapping from its input space $\mathbb{R}^M_t$ to its output space $\mathbb{R}^N_t$. Before training, the owner of $f_t$ randomly initializes the parameters of $f_t$, and embeds the parameters of EPH based on the approach discussed above. The owner then trains $f_t$ on its training dataset $D_t$. During the training process of $f_t$, the owner freezes the parameter space of EPH and only updates the rest of the parameter space. In this way, the parameter space of EPH remains unchanged while other parameters of $f_t$ are updated during training. Note that the loss function of $f_t$ remains unchanged during the training process.

\vspace{-3pt}
\subsection{Ownership Verification}
\label{subsec:Ownership Verification}
Given a model $f_{suspect}$, the owner first extracts the parameter space $EPH_{retrieved}$ from $f_{suspect}$. A straightforward extraction method is to repeat Algorithm \ref{alg:Position-injected} in Section \ref{subsec:Watermark Embedding}. Based on the original HufuNet kept by the owner, he/she can compute the locations in $f_{suspect}$ where EPH is supposedly embedded, and retrieve the corresponding parameter space as $EPH_{retrieved}$. Then the owner merges $EPH_{retrieved}$ with the preserved SPH to obtain $HufuNet_{combined}$. If $f_{suspect}$ is stolen from $f_{wm}$, the rebuilt $HufuNet_{combined}$ is expected to maintain a high accuracy on the standard test set $D_{s\_TEST}$, which has the same distribution as the standard training dataset $D_{s}$. Specifically, the owner evaluates the accuracy $Acc_{combined}$ of $HufuNet_{combined}$ using $D_{s\_TEST}$. If the adversary does not retrain $f_{suspect}$, $Acc_{combined}$ will have the same value as the accuracy of the original HufuNet (i.e., $Acc_{ori}$). Otherwise, $Acc_{combined}$ would drop. To solve this problem, we compare $Acc_{combined}$ with $Acc_{ori}$ using $Diff_{Acc} = |Acc_{ori} - Acc_{combined}|/Acc_{ori}$, if $Diff_{Acc} < \tau_{acc}$, we think that $f_{suspect}$ infringes the IP of the DNN-watermarked $f_{wm}$. $\tau_{acc}$ is the threshold controlling the difference between $Acc_{ori}$ and $Acc_{combined}$. In our evaluation, we find that HufuNet is highly robust against model pruning, fine-tuning and kernels cutoff. Taking CNN as an example, even if the accuracy of $f_{suspect}$ drops by 50.74\%, $Acc_{combined}$ can still be higher than 80\% and $Diff_{Acc}$ is 13.34\% (details are in Section~\ref{subsec:Robustness}). Therefore, we define $\tau_{acc}$ as 15\% in our evaluation, which is good enough to preserve good robustness and integrity of HufuNet.

\subsection{Restore before Retrieve}
\label{subsec:restore}
%\shengzhi{Pay attention here. I reorganized the restore approach as a separate subsection. Check all ref to see if any needs update.}
As a parameter level watermark, HufuNet may suffer from the functionality-equivalent attacks as discussed in Section \ref{sub:destructing}. Therefore, even if $Diff_{Acc}$ is larger than $\tau_{acc}$, a model can still be suspicious ($f_{suspect}$) if it has exactly the same or quite similar structure as the protected model, e.g., the same number of layers and the same number of parameters (with different order) on each layer, or the same number of layers and the same number of kernels on most layers. In such scenarios, we examine $f_{suspect}$ further using the following restore approach and determine whether or not such model has been intentionally adjusted to evade our parameter level watermark. Note that if $f_{suspect}$ is an innocent model, the restore approach will not falsely claim ownership over it.

Regarding structure adjustment, we recover the order of input/output channels of $f_{suspect}$ according to the locally kept HufuNet $f_{wm}$. We start from the first layer where only the order of the output channels can be changed. We compare the parameters of each output channel of $f_{suspect}$ with those of $f_{wm}$ using cosine similarity, so as to find the optimal match.
%to find which one output channel's parameters of $f_{wm}$ has the maximum cosine similarity with the output channel's parameter of $f_{suspect}$. The position of output channel of $f_{wm}$ with the maximum cosine similarity is where the output channel of $f_{suspect}$ that should be. 
In this way, we can recover the order of each output channel of the first layer in $f_{suspect}$ according to  that of our locally stored $f_{wm}$. Then the input channels of the second layer can be restored straightforwardly based on the restored order of the output channels of the first layer. Similarly, the output/input channels of all other layers can be restored accordingly based on the locally kept $f_{wm}$, thus enabling correct retrieval of $EPH_{retrieved}$ even if $f_{suspect}$ experienced structure adjustment. The above cosine similarity approach also works well when many parameters in output channels are adjusted, such as fine-tuning (detailed discussion in Appendix \ref{analysis_of_channel_expansion_principle}).

Regarding parameter adjustment, we first ensure that the order of the input/output channels of $f_{suspect}$ is recovered using the approach described above. Then we perform Singular Value Decomposition (SVD) on each convolution kernel of $f_{suspect}$ and $f_{wm}$ to obtain intermediate singular value matrices. For each pair of singular value matrix in $f_{suspect}$ and singular value matrix in $f_{wm}$, we divide each element of the former by each element of the latter; thus we get a series of resultant matrices. The values on the diagonal of each resultant matrix are averaged to compute the scale factor $c$, used to obtain the restored convolution kernel (i.e., dividing each element in the corresponding convolution kernel $f_{suspect}$ by $c$). We utilize this method to restore all the convolution kernels.

Note that the scale factor is not computed by (i) dividing each element of the convolution kernel in $f_{suspect}$ by each element of the convolution kernel in our local $f_{wm}$, and (ii) computing the average value of the resultant matrix. This is because the singular values of a convolution kernel represent the scaling characteristics of the kernel; it is more reliable to compute the scaling factor from the singular values rather than from kernel parameters directly. This is clear in the case where an attacker first fine-tunes a stolen model and then perform the functionality-equivalent attack through parameter adjustment. The fine-tuning typically makes those smaller values in the convolution kernel change more significantly than those larger ones (e.g., increasing from 1 to 2 results in the factor of 2, but increasing from 10 to 11 yields the factor of 1.1).

Meanwhile, a highly suspicious model $f_{suspect}$ may show minor structural differences, e.g., the number of kernels on one or several layers of $f_{suspect}$ is smaller or larger than those of our watermarked model. We further examine whether or not some kernels of such model have been intentionally cut off or supplemented to evade our watermark. %Note that if $f_{suspect}$ is an innocent model, the approach will not falsely claim ownership over it. First, we also restore the structure of $f_{suspect}$ using cosine similarity approach presented above, since kernels cutoff attack always changes the order of kernels as well, unless all the cutoff kernels are the last ones of the layer. With all the kernels of $f_{suspect}$ restored and our locally stored $f_{wm}$ as a reference, we supplement missing (cutoff) kernels with all parameters as 0. Note that using the values of the corresponding kernels in $f_{wm}$ to supplement may cause false positive on innocent models. 
First, we still restore the structure of $f_{suspect}$ using cosine similarity approach presented above, since kernels cutoff/supplement attacks always change the order of kernels as well, unless all the cutoff/supplemented kernels are the last ones of the layer. With all the kernels of $f_{suspect}$ restored and our locally stored $f_{wm}$ as a reference, we fill in missing (cutoff) kernels with all parameters as 0 or cut off extra (supplemented) kernels directly. Note that using the values of the corresponding kernels in $f_{wm}$ to fill in may cause false positive on innocent models.
%We will add the same number of kernels as output channels cut off to the position of unmatched kernels in $f_{suspect}$, all parameters in these added kernels are 0. Meanwhile, we add some kernels with all 0 parameters to the input channels of the next layer of $f_{suspect}$ according to the position of the output channels cut off in the previous layer, so that the number of input/output channels are same as in $f_{wm}$. After we restore all kernels, we can extract watermarking kernels correctly.
In this way, we can restore $f_{suspect}$ with the same structure as $f_{wm}$ and the same number of kernels $N$, so Algorithm \ref{alg:Position-injected} can be used to extract EPH.

%We still start from the first layer, compare the cosine similarity between each kernel in the $f_{cut}$ and each kernel in the local model $f_{wm}$, each kernel of $f_{cut}$ is placed at the position of some kernel in $f_{wm}$'s kernel, which has the greatest cosine similarity to this kernel in $f_{cut}$. In this way, after matching the positions of all kernels in $f_{cut}$, those unmatched kernels in $f_{wm}$ are actual cut kernels in $f_{cut}$. We will add the same number of kernels as cut kernels to $f_{cut}$, all parameters in these added kernels are 0. These added kernels are placed in the position of cut kernels. In this way, the number and order of kernels in the first layer is restored as same as the local $f{wm}$. Meanwhile, we add some kernels with all 0 parameters to the input channels of the second layer of $f_{cut}$ according to the position of the output channels cut in the first layer, so that the number/order of input channels of second layer in $f_{cut}$ are same as in $f_{wm}$. Similarly, the output/input channels of all other layers can be restored accordingly based on the locally kept $f_{wm}$. In the end, the number of kernels N and order in $f_{cut}$ will be the same as $f_{wm}$, we can extract watermarking kernel correctly.}


\begin{comment}
The owner can verify his/her ownership by comparing the performance of $HufuNet_{combined}$ against a threshold $\tau_{acc}$ defined below:
\begin{equation}
\label{formulatao}
\small
\tau_{acc} = \begin{cases}
& 0.85 \qquad \qquad \qquad \qquad ACC_{HufuNet_{combined}} \geq 0.85  \\ 
& e^{-|ACC_{f_{suspect}}-{ACC_{f_{wm}}}|} \cdot ACC_{HufuNet} \qquad \quad else
\end{cases}
\end{equation}
where $ACC_{f_{suspect}}$, $ACC_{f_{wm}}$, and $ACC_{HufuNet}$ are the accuracy of the suspect model $f_{suspect}$, the DNN-watermarked model $f_{wm}$, and the original HufuNet, respectively. In the case that the accuracy of $HufuNet_{combined}$ itself is greater or equal to 85\%, we are confident to claim the ownership over the suspect model directly by setting the threshold $\tau_{acc}$ just as $0.85$. \kai{how to choose this value?} Otherwise, a penalty factor is used to adjust the accuracy of original HufuNet in computing the threshold, since the adversaries may have significantly pruned and/or fine-tuned $f_{wm}$ to obtain their DNN model $f_{suspect}$, thus destructing the watermark EPH accordingly. 
\end{comment}


%The owner can verify his/her ownership by comparing the performance of $HufuNet_{combined}$ against a threshold $\tau_{acc}$. After many experiments, we find that under the premise of ensuring the complete function of the main task of the DNN-watermarked model, the accuracy of $HufuNet_{combined}$ will not be lower than $80\%$, so we set the threshold $\tau_{acc}$ to $80\%$. If the accuracy of $HufuNet_{suspect}$ on $D_{s\_TEST}$ is no less than the threshold $\tau_{acc}$, the owner may claim that $f_{suspect}$ infringes the IP of the DNN-watermarked $f_{wm}$.

%The penalty factor is the exponential power of $e$, with the power equal to the negative of the absolute value of the difference between the accuracy of the preceding two models, which indicates the scale of revision. If the accuracy of $HufuNet_{suspect}$ on $D_{s\_TEST}$ is no less than the threshold $\tau_{acc}$, the owner may claim that $f_{suspect}$ infringes the IP of the DNN-watermarked $f_{wm}$. 

%\subsection{Fulfilling Design Requirements}
%\label{subsection:Analysis of Property of HufuNet}
%\noindent\textbf{Stealthiness and Security.} The ownership verification of HufuNet depends on its reconstruction, security against forging ,and robustness against revision. Given a DNN-to-be-protected, several layers are selected from the middle and back of the model in a hash way to embed our watermark. For each chosen layer, the parameter space of each CNN layer in EPH is also embedded inside in a hash way. Hence, the way to retrieve the $Embedded\ Piece\ of HufuNet_{retrieved}(EPH_{retrieved})$ is a secret to the owner only. \lpz{It is impossible for an attacker to obtain our key of HMAC, so he cannot know exactly where we embed EPH, which guarantees stealthiness.} Meanwhile, we did not introduce extra regular items to the loss function during the training process, so the variance of parameters on each layer will not increase significantly (Refer to experimental results in Section \ref{exp_stealthiness}). Hence, the statistical approach~\cite{wang2019attacks} against white-box watermarks cannot find our EPH. Moreover, SPH is kept as another secret and only known to the owner. Overall, the reconstruction of HufuNet is based on two secrets: the way to retrieve $EPH_{retrieved}$ and the record of the EPH, which are quite difficult, if not impossible, for attackers to obtain. Even aware of the details of our watermarking approach, forging HufuNet is still challenging for attackers, which guarantee security. 

%\noindent\textbf{Robustness.} Since the attackers usually prune and/or fine-tune a stolen DNN model before reusing it, EPH needs to be robust against such revision to the DNN-watermarked. A largely tampered EPH, together with SPH, cannot fulfill the desired classification task for ownership verification. The robustness of EPH against pruning and fine-tuning lies in the parameter redundancy in DNN models. We find that usually the top 50\% parameters ranked using their absolute values contribute most to the specific task of the DNN models, while other parameters with relatively small absolute values can be considered as ``redundancy'' in the parameter space, mainly optimizing the models. Hence, if the parameters with larger absolute values in the EPH do not change significantly, HufuNet should be robust on its classification task. 

%Model pruning trims down the not so important parameters, typically those with small absolute values, to preserve the capability of its main task. The attackers can apply pruning on the DNN-watermarked, to trim down parameters with small absolute values in the entire parameter space of DNN-watermarked. Fortunately, most of the parameters in EPH are at the higher range of the entire parameter space of DNN-watermarked in terms of absolute values, thus evading the model pruning. The reason for that is as below: EPH includes well-trained CNN layers, which when embedded, can help the training of DNN-watermarked quickly converges as discussed in Section \ref{subsec: watermark_Genaration}. Therefore, most of the parameters of the EPH should pay a leading role in the main task of the DNN-watermarked, thus with larger absolute values, which is consistent with what we observed during experiments. Similarly, model fine-tuning has little impact on the parameters with larger values, thus the parameter space of EPH can mostly be preserved. The experimental results in Section \ref{subsec:Robustness} demonstrates the robustness of HufuNet. 

\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Justification of Design}
\label{subsec:justification}
\noindent\textbf{Model fine-tuning and pruning}
The model owner embeds watermark EPH into the convolutional layers of DNN-to-be-protected $f_t$. After stealing the model $f_{wm}$, an adversary may initialize all its convolutional layers and retrain them. However, this would demand extensive computing resources and a large amount of training data, which violates our threat model as such adversary is capable of training $f_t$ from scratch without the motivation of stealing it from $f_{wm}$. Instead, an adversary may fine-tune the convolutional layers and prune uncritical neurons of $f_{wm}$, hoping to remove the ``footprint'' of any watermark without compromising its main task.

Due to the stealthiness (evaluated in Section \ref{exp_stealthiness}) and small scale of EPH in DNN-watermarked (EPH consumes 1.48\%$\sim$3.44\% of the parameter space of CNN models, and 13.38\% of the parameter space of the LSTM model,
%\lpz{typically around 3.28\%(on average VGG11, GoogLeNet, Resnet18, Resnet34), also we test little model LSTM embedded with our EPH around 13.38\%} 
based on our experiment in Section \ref{subsec:Performance}), it is difficult for model pruning and fine-tuning to destroy the embedded watermark. The robustness of EPH against pruning and fine-tuning is also attributed to the parameter redundancy in DNN models. Usually a portion of parameters (e.g., the top 50\% parameters with large absolute values) contributes most to the task of a DNN model, while the other parameters can be considered ``redundant'' in the parameter space, making minor contribution to the model's task. Model retraining mainly affects those not-so-important values in the parameter space of DNN-watermarked; otherwise, the performance of the retrained model would be significantly worse than the watermarked model, which defeats the purpose of ownership verification. As long as a majority of significant parameters in EPH remains stable in model retraining, ownership verification can be performed robustly. We discover that this is the case in our rigorous experiments (refer to Section \ref{sec:Evaluation} for details). 


\noindent\textbf{Watermark forging.}
An intuitive idea is that an adversary forges a valid HufuNet-style watermark from the public dataset $D_s$ and embeds it into DNN-watermarked. In particular, the adversary first trains a HufuNet from $D_s$; he/she then chooses a secret key and embeds EPH from the forged HufuNet into DNN-watermarked following the watermark embedding algorithm. In case of ownership dispute, the adversary may perform ownership verification on his/her stolen model from which the forged watermark can be detected following the ownership verification algorithm. In such a case, the adversary's secret key would be different from the owner's secret key with an overwhelming probability; therefore, it is highly unlikely that the adversary's forged watermark overwrites the owner's watermark in DNN-watermarked. Consequently, the adversary can only present a model with both the adversary's watermark and the owner's watermark detected, while the owner of the model can present the original DNN-watermarked with only the owner's watermark detected. It is thus clear who is the true owner to resolve the dispute.

Therefore, the adversaries have to leverage the existing parameters in the stolen model, rather than revising any. Meanwhile, two requirements have to be satisfied to forge a valid and effective HufuNet-style watermark: (R1) the accuracy of the forged HufuNet passes the threshold; (R2) the positions where the embedded kernels (EPH) are retrieved should satisfy the correlation based on Line 3 in Algorithm \ref{alg:Position-injected}. Below we discuss two different watermark forging attacks depending on which requirement to satisfy first: first accuracy then correlation and first correlation then accuracy. 

\textit{First accuracy then correlation.} Since both the training dataset $D_s$ and the testing dataset $D_{s\_TEST}$ are standardized for training and verifying HufuNet (see Section \ref{subsec: watermark_Genaration}), the adversaries cannot forge a valid HufuNet with arbitrary datasets. However, it does not rule out the possibility of forging a valid HufuNet from the public dataset $D_s$ with high accuracy. It is possible that the parameter space of DNN-watermarked is large and includes sufficient values required by an adversary to match a forged HufuNet. However, to prevent the adversaries from associating the matched values between DNN-watermarked and a forged HufuNet, our embedding algorithm computes the embedding location of each EPH kernel in DNN-watermarked based on a secret key, the parameter values of the EPH kernel, and its index through a secure HMAC function. It is computationally tricky for the adversaries to discover an appropriate secret key that can associate the matched values based on our evaluation results in Section \ref{subsec:security1}. 

\textit{First correlation then accuracy.} Since Algorithm \ref{alg:Position-injected} is public, the adversary can randomly select a key, test each kernel in the stolen model based on Line 3 in Algorithm \ref{alg:Position-injected}, and try to find all the kernels that satisfy the correlation. The adversary can explore quite a number of different keys, e.g., 1,000, and check which key finds the most kernels that satisfy the correlation. With enough such kernels found based on a particular key, the adversary can claim those kernels are his/her EPH. To forge a valid HufuNet-style watermark, the adversary simply places those kernels into the convolution layers, randomly initializes a fully connected layer, and trains the fully connected layer using the public dataset $D_s$. Such watermark should have high accuracy on the public testing dataset as well. However, it is extremely difficult, if not impossible, to locate a random key that can find enough kernels that satisfy the correlation to construct the convolution layers of a model based on our evaluation results in Section \ref{subsec:security1}. Note that brute force searching of all possible keys may let the adversary obtain our key used to embed our HufuNet, but it is computationally hard to traverse all the keys (a key of 64 byte long means 2$^{256}$ different keys in total.). 

%\lpz{The second way is that since Algorithm 1 is public, the adversary can randomly select a secret key, and search for index of all kernels in the stolen NN as Algorithm 1. If there are tens of thousands kernels' hash results matching with their true index, adversary think these kernels as watermarking ones that true owner former embedding. This can be done by brute force searching. After finding such kernels, we assume adversary may know the structure of HufuNet, they will place all these found kernels to convolution layers. Then the attacker can randomly initializes a fully connected layer after the watermarking kernels, train the fully connected layer using the public training dataset and get forged HufuNet. The forged HufuNet will have high accuracy on the public testing dataset to verify ownership.}



%Since the key to compute the hash and the parameter values of HufuNet are kept as a secret, there is no way for adversaries to learn the locations where we embed EPH, thus impossible to steal it. Moreover, SPH is kept as another secret and only known to the model owner, which is also out of reach of adversaries. Note that since we need to compute the hash to obtain the embedding locations during ownership verification, EPH also needs to be preserved. Therefore, we can always have a local copy of the original parameter values of each convolution kernel as the input to the hash function, because those values from the suspect model could have been changed due to fine-tuning or pruning.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}


==> arxiv2021 HufuNet/sections/Background.tex <==
\section{Background}
\label{sec:Background}
%In this section, we give background on deep neural networks, digital watermarking and watermark destructing approaches.

\ignore{\subsection{Deep Neural Networks}
A neural network can be viewed as a mapping function $f: \mathbb{R}^M \rightarrow \mathbb{R}^N$ given a training dataset $D_{tr} = \{(x^1_{tr}, y^1_{tr}), \cdots, (x^n_{tr}, y^n_{tr})\}$, where $x^i_{tr} \in \mathbb{R}^M$, $y^i_{tr} \in \mathbb{R}^N$. If it is well trained, $f$ should output $y^i$ with a high probability for the input $x^i$. Function $f$ can be computed based on a weight vector $w$ organized in a network structure, where the weight values are determined in the training process using the training data $D_{tr}$. If the structure of a neural network consists of multiple layers, it is usually called a deep neural network (DNN). DNN is the foundation of many AI applications, which drives the rapid development of speech and image recognition, natural language processing, autonomous driving, medical diagnosis, etc. It is usually highly costly to train a DNN model due to the resources it consumes, including a large amount of high-quality training data, high-performance computing facilities, as well as domain experts for designing network structures and training parameters. Therefore, it is necessary to protect the IP of DNN models using techniques such as digital watermarking. }


\subsection{Digital Watermarking}
Digital watermarking is a content-based, information hiding technique for embedding/detecting digital information into/from carrier data (e.g., multimedia, documents, software, databases, etc.). It is desired that the embedded watermark should not impact the regular use of carrier data, and be difficult to be detected or removed. Recently, digital watermarking has been applied to the protection of DNN models, and can be classified into white-box approaches and black-box approaches. The white-box approaches assume that the owner of a DNN model can access the ``internals'' of a suspect model to verify the ownership of the model. For instance, Uchida et al. use a parameter regularizer to embed a watermark, which is a matrix of parameters, into the target model’s parameter space during its training process. When verifying ownership over a suspect model, the owner retrieves the matrix from the model, computes the retrieved matrix's product and a pre-generated key vector, and compares the result with a local secret kept by the owner~\cite{uchida2017embedding}.

In contrast, black-box watermarking approaches mostly rely on probing a suspect model for ownership verification, thus relaxing the requirement of the internal knowledge of the suspect model. Black-box watermarking approaches can further be categorized into two classes, blind~\cite{li2019prove,namba2019robust} approaches and non-blind approaches~\cite{adi2018turning,guo2018watermarking,zhang2018protecting,rouhani2018deepsigns}, depending on whether or not an embedded watermark can be perceived by the human visual system~\cite{li2019prove}. 

Most black-box watermarking schemes are implemented based on embedding backdoors~\cite{chen2017targeted,gu2017badnets} into the target DNN models. Embedding a backdoor into a neural network model is to deliberately train the model using a training dataset that is augmented with certain specific inputs (i.e., triggers) and their desired labels (typically wrong labels), which should be selected uniquely by the model's owner and thus demonstrate the model's distinguishable behavior. Once trained, the model should output the desired labels for the specific inputs. The mapping between the specific inputs and their desired labels is considered as a backdoor, and used as a watermark. The specific inputs are kept as a secret by the model's owner. The model's owner can claim his/her ownership over a suspect model if the backdoor/watermark is detected in the sense that the model outputs the desired labels given the specific inputs from the owner's secret. However, recent research indicates that most backdoor-based watermarks are vulnerable to be detected and destroyed~\cite{chen2018detecting,liu2018fine,wang2019neural}.

\subsection{Watermark Destructing Approaches}
\label{sub:destructing}
\noindent\textbf{Entire model retraining.} The most effective method to destruct an embedded watermark in a model is to retrain it completely. However, since such entire model retraining typically requires similar amount of expertise, effort, training data and computing power as training their own model from scratch, adversaries would rather train their own model than stealing to avoid any potential legal issues.  
%\noindent\textbf{Selective layer retraining.} Constrained by limited computing power and/or training dataset available, adversaries might randomly select one layer from the stolen model, initialize all the parameters of the layer and retrain them to destruct any embedded watermark. Compared with retraining the entire stolen model or training their own model from fresh, this is more economic and reasonable for adversaries, and a watermark, if any in the stolen model, is highly likely destructed.

\noindent\textbf{Fine-tuning.} Fine-tuning is typically used to optimize an already-trained DNN model to augment it with additional tasks or reinforce its performance. Fine-tuning involves an update to the parameter values in the model, thus possible destroying the embedded watermark. Generally, the scale of fine-tuning is flexible, depending on the training dataset and computing power available. Therefore, adversaries can fine-tune the stolen model according to their capacity to destruct the watermark.

\noindent\textbf{Pruning.} Model pruning approach is commonly used for model compression to produce smaller, more memory-efficient and power-efficient models with negligible loss inaccuracy. Typically, it prunes less-connected, unimportant neurons in the neural network by zeroizing them without changing the network structure. Model pruning can be used by those adversaries lack of training power to destruct the embedded watermark in their stolen model, since it does not involve any retraining.

\noindent\textbf{Functionality-equivalent attack.} Functionality equivalent attack can be launched via structure adjustment and parameter adjustment. The attackers do not need any training resources or training dataset to retrain the model. Instead, they can simply reorder the sequence of output channels on one convolution layer, and adjust the corresponding sequence of input channels on the next convolution layer to obtain a functionality-equivalent model (called structure adjustment in this paper), due to the isomorphism of many CNN structures. Furthermore, if the stolen DNN model is with ReLU as the activation function, the attackers can also scale the weights of all the neurons on one layer by a positive constant $c \textgreater 0$, and then scale the next layer by $1/c$ to get a functionality-equivalent model (called parameter adjustment in this paper) to destruct embedded watermarks. Functionality-equivalent attack can also be launched via channel expansion. In particular, adversaries randomly choose two adjacent layers of their stolen model with matrices $A$ and $B$. Then they increase the output dimension of $A$ (by increasing its output channels) to get $A'$, and $B$ to get $B'$, with the restriction of $(A' B') x = (A B) x$, where $x$ is the feature map propagated in neural networks. Finally, the adversaries can further apply structure adjustment or fine-tuning to undermine the embedded watermarks.

%Functionality equivalent attack can be launched via structure adjustment and parameter adjustment. The attackers do not need any training resources or training dataset to retrain the model. Instead, they can simply reorder the sequence of output channels on one convolution layer, and adjust the corresponding sequence of input channels on the next convolution layer to obtain a functionality-equivalent model (called structure adjustment in this paper), due to the isomorphism of many CNN structures. Furthermore, if the stolen DNN model is with ReLU as the activation function, the attackers can also scale the weights of all the neurons on one layer by a positive constant $c \textgreater 0$, and then scale the next layer by $1/c$ to get a functionality-equivalent model (called parameter adjustment in this paper). The adversary can also try such functionality-equivalent attack on the stolen model to destruct embedded watermarks. 

\noindent\textbf{Kernels cutoff and supplement.} The adversary can cut off (completely remove some kernels, rather than zeroizing them as pruning) or supplement some kernels in the stolen model to obtain a new model with similar performance but different number of kernels and structure. To ensure similar performance as the stolen model, the adversary should cut off or supplement kernels carefully: if some output channels (kernels) of one layer are cut off or supplemented, then the corresponding input channel of the next layer should also be cut off or supplemented. Besides, since kernels cutoff will reduce the performance of the model, the adversary may not want to cut off too many kernels from the stolen model. Kernels cutoff or supplement can also be leveraged by the adversary to destruct embedded watermarks. %The adversary can also supplement some kernels in the stolen model. Similar as kernels cutoff, if some output channels of one layer are supplemented, then the corresponding input channel of the next layer should also be supplemented. 

%\noindent\textbf{Fraudulent Ownership Claim.} If watermarked DNN models are stolen by model prowlers, they may analyze the models, generate forged watermarks, and claim fraudulent ownership over the stolen models. In the white-box case, model prowlers are assumed to have full access to the watermarked models, be proficient in machine learning, and understand DNN watermarking scheme. 

%\noindent\textbf{Evasion Attack.} Evasion attack refers to attack towards the black box state-of-the-art watermarking technique presented in [], which aims to avoid backdoor-based watermark verification in black box situation. In general, non-blind is generally vulnerable to evasion attack, previous studies based on non-blind watermark either fail to defend against the evasion attack or have not explicitly dealt with fraudulent claims of ownership by adversaries. However, watermark framework based on blind-watermark to embed the watermark is robust against to evasion attack[].

==> arxiv2021 HufuNet/sections/Conclusion.tex <==
\vspace{12pt}
\section{Conclusion}
\label{sec:Conclusion}
%-------------------------------------------------------------------------------

In this paper, we proposed HufuNet, a robust and secure watermarking approach, to protect DNN models' ownership. We divided HufuNet into two pieces, with the left piece EPH embedded into the DNN-to-be-protected and the right piece SPH kept locally as the secret to verify ownership of suspect DNN models. Compared with previous watermark approaches, the ownership verification of HufuNet is more robust against model fine-tuning, pruning and is more secure against watermark forging, which is demonstrated by our experimental results conducted on five popular DNN models. Meanwhile, our watermarking approach has a negligible impact on the performance of the DNN models it protects. It is robust to kernel cutoff/supplement, adaptive to the functionality-equivalent attack, and does not falsely claim ownership on innocent models.

==> arxiv2021 HufuNet/sections/Evaluation.tex <==
\section{Evaluation}
\label{sec:Evaluation}
%-------------------------------------------------------------------------------
%We evaluate the effectiveness of HufuNet in the following aspects: robustness, adaptiveness, stealthiness, security, integrity and fidelity, consistent with the design requirements in Section \ref{Design_Requirements}. Below in this section, we present the experimental results.

%------------------------------------------------------------------%
%------------------------------------------------------------------%
Based on the watermark destruction approaches discussed in Section \ref{sub:destructing}, we evaluate our solution in the following aspects. (i) robustness: watermarks should still be detected by owners from stolen DNN models even if the models experienced fine-tuning, pruning and kernels cutoff/supplement (refer to Section \ref{subsec:Robustness}); (ii) adaptiveness: watermarks should still be detected by owners even if the model has been converted to a functionality-equivalent one via structure adjustment, parameter adjustment or channel expansion (refer to Section \ref{subsec:adaptiveness}); (iii) against synthetic attacks: watermark can still be detected by owners even if the attackers applied fine-tuning, pruning and functionality-equivalent attacks together on their stolen models (refer to Section \ref{subsec:combination adaptiveness with robustness}); (iv) stealthiness: it is difficult for attackers to learn the existence of watermark from a stolen DNN model (refer to Section \ref{exp_stealthiness}); (v) security: it is difficult for attackers to forge a valid watermark for a stolen DNN model (also called ambiguity attack~\cite{fan2019rethinking}, refer to Section \ref{subsec:security1}); (vi) integrity: it is highly unlikely for DNN owners to claim ownership over innocent DNN models (refer to Section \ref{subsec:integrity}); and (vii) fidelity: watermark-embedding should impact little on the performance of the original DNN models (refer to Section \ref{subsec:fidelity}).

\subsection{Experimental Setup}
\label{subsec:Experiment Setting}

%\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 

\noindent\textbf{Models}. Without loss of generality, we conduct experiments on five models: VGG11~\cite{simonyan2014very}, GoogLeNet~\cite{szegedy2015going}, Resnet18 and Resnet34~\cite{he2016deep}, and LSTM~\cite{hochreiter1997long}, which are all used as DNNs-to-be-protected. HufuNet is designed with five convolutional layers (used as EPH) and one fully connected layer (used as SPH).

%\noindent\textbf{Models}. Without loss of generality, we conduct experiments on five models: VGG11~\cite{simonyan2014very}, a deep convolutional network by Oxford Visual Geometry Group, which contains eight convolutional layers and three fully connected layers; GoogLeNet~\cite{szegedy2015going}, a deep convolutional neural network proposed by Google; Resnet18 and Resnet34~\cite{he2016deep}, a deep residual neural network; LSTM~\cite{hochreiter1997long}, a time recurrent neural network architecture, which is to process and forecast important events with very long intervals and delays in time series. They are all used as the DNNs-to-be-protected. HufuNet is designed to include five convolutional layers (used as EPH) and one fully connected layer (used as SPH).

\noindent\textbf{Datasets}. We choose four datasets: Fashion-MNIST~\cite{xiao2017fashion}, IMDB~\cite{maas-EtAl:2011:ACL-HLT2011}, CIFAR-10, and CIFAR-100 ~\cite{krizhevsky2009learning} for the above five models accordingly. 
%Fashion-MNIST is a dataset of Zalando's article images consisting of a training set of 60,000 samples and a testing set of 10,000 samples. Each sample is a $28 \times 28$ gray-scale image, associated with a label of 10 classes. IMDB is a dataset for binary sentiment classification containing substantially more data than previous benchmark datasets, which provide a set of 25,000 highly polar movie reviews for training and 25,000 for testing. CIFAR-10 consists of $32 \times 32$ color images in 10 classes, with 5,000 training images and 1,000 testing images per class. CIFAR-100 is similar to CIFAR-10, except it contains 100 classes, with 500 training images and 100 testing images per class. 
We use Fashion-MNIST to train our HufuNet, CIFAR-10 to train VGG11, GoogLeNet as well as Resnet18, CIFAR-100 to train Resnet34, and IMDB to train LSTM as shown in Table \ref{tab:datasets} in Appendix. The classification task and the main task of the DNN models are used interchangeably thereafter.

\noindent\textbf{Platform}. All our experiments are conducted on a server running 64-bit Ubuntu 18.04 system with Intel Xeon E5-2620 v4 @ 2.10GHz CPU, 128GB memory, 3TB hard drive and 3 Nvidia GPU TiTan X GPUs each with 12GB memory.

%------------------------------------------------------------------%
%------------------------------------------------------------------%


\vspace{-8pt}
\subsection{Baseline Performance}
\label{subsec:Performance}
We evaluate the ownership verification of HufuNet on the model without any changes between embedding and verifying, i.e., assuming adversaries just steal the model without performing any other operations on the stolen model, as the baseline performance. The number of parameters of the five DNNs-to-be-protected and HufuNet are shown in Table \ref{tab:parameter} in Appendix. It can be seen that our watermark EPH only consumes a small portion of the parameter space of VGG11, GoogLeNet, Restnet18 and Resnet34, ranging from {1.48}\% to {5.37}\%), since the number of parameters of these four models are relatively large. Since LSTM is intentionally selected to evaluate the performance of HufuNet on smaller models, EPH consumes up to 13.38\% of its parameter space, considering LSTM only contains 9,251 KB parameters in just three layers.

\begin{table}
\begin{threeparttable}
\centering
\footnotesize
\caption{Baseline Performance of Ownership Verification}
\label{tab:Performance of ownership verification}
\begin{tabular}{m{1.0cm}
<{\centering}|m{0.8cm}
<{\centering}|m{1.3cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.0cm}
<{\centering}|m{0.7cm}
<{\centering}}
\hline
\textbf{ }& \textbf{VGG11}& \textbf{GoogLeNet}& \textbf{Resnet18}& \textbf{Resnet34}& \textbf{LSTM}\\
\hline \hline
\textbf{Original$^{1}$} & \text{77.77$\%$} &\text{90.85$\%$}& \text{86.14$\%$}&\text{70.20$\%$}& \text{87.08$\%$} \\ \hline
\textbf{Suspect$^{2}$} & \text{77.77$\%$} &\text{90.85$\%$}& \text{86.14$\%$}&\text{70.20$\%$}& \text{87.08$\%$} \\ \hline
\textbf{$\tau_{acc}^{3}$}& \text{15$\%$} &\text{15$\%$}& \text{15$\%$}&\text{15$\%$}& \text{15$\%$} \\ \hline
\textbf{Combine$^{4}$}& \text{92.32$\%$} &\text{92.32$\%$}& \text{92.32$\%$}&\text{92.32$\%$}& \text{92.32$\%$} \\ \hline
\end{tabular}
\begin{tablenotes}
\item[1] Original indicates the accuracy of the original DNN-watermarked. 
\item[2] Suspect indicates the accuracy of the suspect model we would like examine. Since there is not any kind of retraining conducted, it demonstrates the same accuracy as that of our DNN-watermarked. 
\item[3] The threshold $\tau_{acc}$ is set as 15\%, so $HufuNet_{combined}$ accuracy above 80\% indicates ownership verification according to Section \ref{subsec:Ownership Verification}.
\item[4] Combine indicates the accuracy of the $HufuNet_{combined}$. Since there is not any kind of retraining conducted, it demonstrates the same accuracy as that of our original HufuNet. 
\end{tablenotes}
\end{threeparttable}
\end{table}

%--------------------------------------------------------------------------%
%--------------------------------------------------------------------------%

\begin{table*}[h]
\centering
\footnotesize
\caption{Robustness against Fine-tuning}
\label{tab:Robustness against Finetuning}
\begin{tabular}{m{0.7cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}}

\hline
\multirow{2}{*}{\textbf{\makecell[c]{Epochs}}} & \multicolumn{2}{c|}{\textbf{VGG11}}& \multicolumn{2}{c|}{\textbf{GoogLeNet}}& \multicolumn{2}{c|}{\textbf{Resnet18}}&\multicolumn{2}{c|}{\textbf{Resnet34}}& \multicolumn{2}{c}{\textbf{LSTM}}\\ \cline{2-11}
\text{}&\textbf{DNN-watermarked}&\textbf{HufuNet}&\textbf{DNN-watermarked}& \textbf{HufuNet}&\textbf{DNN-watermarked}&\textbf{HufuNet}& \textbf{DNN-watermarked}&\textbf{HufuNet}& \textbf{DNN-watermarked}&\textbf{HufuNet}\\

\hline \hline
\text{0}&\text{77.77$\%$}&\text{92.32$\%$}&\text{$90.85\%$}& \text{$92.32\%$}&\text{$86.14\%$}&\text{$92.32\%$}&\text{$70.20\%$}&\text{$92.32\%$}& \text{$87.08\%$}&\text{$92.32\%$}\\

\hline
\text{10}&\text{75.35$\%$}&\text{92.37$\%$}&\text{$89.55\%$}& \text{$91.91\%$}&\text{$85.75\%$}&\text{$92.34\%$}& \text{$66.97\%$}&\text{$92.26\%$}& \text{$85.90\%$}&\text{$92.28\%$}\\

\hline 
\text{20}&\text{74.70$\%$}&\text{92.20$\%$}&\text{$89.75\%$}& \text{$91.99\%$}&\text{$85.70\%$}&\text{$92.35\%$}&\text{$66.78\%$}&\text{$92.20\%$}& \text{$86.10\%$}&\text{$92.36\%$}\\

\hline 
\text{30}&\text{72.30$\%$}&\text{92.21$\%$}&\text{$89.75\%$}& \text{$92.03\%$}&\text{$85.60\%$}&\text{$92.36\%$}& \text{$68.19\%$}&\text{$92.15\%$}&\text{$85.60\%$}&\text{$92.18\%$}\\

\hline 
\text{40}&\text{73.65$\%$}&\text{92.16$\%$}&\text{$89.70\%$}& \text{$92.07\%$}&\text{$85.65\%$}&\text{$92.36\%$}& \text{$67.44\%$}&\text{$92.01\%$}& \text{$88.20\%$}&\text{$92.19\%$}\\

\hline 
\text{50}&\text{73.35$\%$}&\text{92.19$\%$}&\text{$89.70\%$}& \text{$92.06\%$}&\text{$85.50\%$}&\text{$92.32\%$}&\text{$67.48\%$}&\text{$91.83\%$}&  \text{$87.80\%$}&\text{$92.22\%$}\\

\hline
\text{60}&\text{75.80$\%$}&\text{92.18$\%$}&\text{$89.80\%$}& \text{$92.04\%$}&\text{$85.50\%$}&\text{$92.39\%$}& \text{$67.64\%$}&\text{$91.88\%$}&\text{$88.00\%$}&\text{$92.17\%$}\\

\hline 
\text{70}&\text{75.80$\%$}&\text{92.16$\%$}&\text{$89.70\%$}& \text{$92.02\%$}&\text{$85.55\%$}&\text{$92.37\%$}&\text{$67.51\%$}&\text{$91.85\%$}& \text{$87.30\%$}&\text{$92.11\%$}\\

\hline 
\text{80}&\text{75.85$\%$}&\text{92.16$\%$}&\text{$89.65\%$}& \text{$92.01\%$}&\text{$85.70\%$}&\text{$92.39\%$}&\text{$67.81\%$}&\text{$91.53\%$}& \text{$87.50\%$}&\text{$92.14\%$}\\

\hline
\text{90}&\text{75.70$\%$}&\text{92.14$\%$}&\text{$89.45\%$}& \text{$92.03\%$}&\text{$85.70\%$}&\text{$92.39\%$}& \text{$66.91\%$}&\text{$91.32\%$}&\text{$87.50\%$}&\text{$92.16\%$}\\

\hline
\text{100}&\text{75.60$\%$}&\text{92.14$\%$}&\text{$89.45\%$}& \text{$92.03\%$}&\text{$85.70\%$}&\text{$92.39\%$}&\text{$67.67\%$}&\text{$91.08\%$}& \text{$87.60\%$}&\text{$92.16\%$}\\

\hline
\end{tabular}
\begin{tablenotes}
\item \text{The HufuNet in the table indicates the accuracy of $HufuNet_{combined}$.}
\end{tablenotes}
\end{table*}

\begin{table*}[h]
\centering
\footnotesize
\caption{Robustness against Pruning}
\label{Robustness against Pruning}
\begin{tabular}{m{0.7cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.42cm}
<{\centering}|m{1.0cm}
<{\centering}}
%HufuNet
\hline
\multirow{2}{*}{\textbf{\makecell[c]{pct.}}} & \multicolumn{2}{c|}{\textbf{VGG11}}& \multicolumn{2}{c|}{\textbf{GoogLeNet}}& \multicolumn{2}{c|}{\textbf{Resnet18}}&\multicolumn{2}{c|}{\textbf{Resnet34}}& \multicolumn{2}{c}{\textbf{LSTM}}\\ \cline{2-11}
\text{}&\textbf{DNN-watermarked}&\textbf{HufuNet}&\textbf{DNN-watermarked}&\textbf{HufuNet}&\textbf{DNN-watermarked}&\textbf{HufuNet}& \textbf{DNN-watermarked}&\textbf{HufuNet}&\textbf{DNN-watermarked}&\textbf{HufuNet}\\

\hline \hline
\text{0}&\text{77.77$\%$}&\text{92.32$\%$}&\text{$90.85\%$}& \text{$92.32\%$}&\text{$86.14\%$}&\text{$92.32\%$}&\text{$70.20\%$}&\text{$92.32\%$}& \text{$87.08\%$}&\text{$92.32\%$}\\

\hline
\text{10$\%$}&\text{77.68$\%$}&\text{92.33$\%$}&\text{$90.77\%$}& \text{$92.29\%$}&\text{$86.14\%$}&\text{$92.29\%$}&\text{$70.29\%$}&\text{$92.27\%$}& \text{$87.06\%$}&\text{$92.33\%$}\\

\hline 
\text{$20\%$}&\text{77.80$\%$}&\text{92.29$\%$}&\text{$90.55\%$}& \textbf{$92.32\%$}&\text{$85.96\%$}&\text{$92.34\%$}&\text{$70.20\%$}&\text{$92.46\%$}& \text{$87.18\%$}&\text{$92.37\%$}\\

\hline 
\text{$30\%$}&\text{77.82$\%$}&\text{92.27$\%$}&\text{$90.19\%$}& \text{$92.32\%$}&\text{$85.75\%$}&\text{$92.35\%$}&\text{$69.70\%$}&\text{$92.20\%$}& \text{$87.26\%$}&\text{$92.36\%$}\\

\hline 
\text{40$\%$}&\text{$77.64\%$}&\text{92.37$\%$}&\text{$85.90\%$}& \text{$92.36\%$}&\text{$82.24\%$}&\text{$92.37\%$}&\text{$67.25\%$}&\text{$91.98\%$}& \text{$86.94\%$}&\text{$92.19\%$}\\

\hline 
\text{50$\%$}&\text{77.23$\%$}&\text{92.29$\%$}&\text{$56.46\%$}& \text{$92.07\%$}&\text{$74.81\%$}&\text{$92.09\%$}&\text{$56.46\%$}&\text{$91.21\%$}& \text{$86.85\%$}&\text{$91.86\%$}\\

\hline
\text{60$\%$}&\text{75.68$\%$}&\text{92.25$\%$}&\text{$19.63\%$}& \text{$91.73\%$}&\text{$46.84\%$}&\text{$91.74\%$}&\text{$27.86\%$}&\text{$89.19\%$}& \text{$86.89\%$}&\text{$91.36\%$}\\

\hline 
\text{70$\%$}&\text{69.84$\%$}&\text{91.86$\%$}&\text{$11.73\%$}& \text{$90.29\%$}&\text{$11.44\%$}&\text{$90.35\%$}&\text{$4.86\%$}&\text{$85.60\%$}& \text{$86.28\%$}&\text{$89.95\%$}\\

\hline 
\text{$80\%$}&\text{50.74$\%$}&\text{90.99$\%$}&\text{$10.00\%$}& \text{$87.63\%$}&\text{$10.00\%$}&\text{$87.80\%$}&\text{$1.10\%$}&\text{$65.61\%$}& \text{$84.16\%$}&\text{$85.74\%$}\\

\hline
\text{$90\%$}&\text{21.74$\%$}&\text{87.54$\%$}&\text{$10.00\%$}& \text{$66.12\%$}&\text{$10.00\%$}&\text{$67.83\%$}&\text{$1.00\%$}&\text{$34.82\%$}& \text{$60.75\%$}&\text{$58.14\%$}\\

\hline
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[*]\text{pct. indicates the percentage of pruning. The HufuNet in the table indicates the accuracy of $HufuNet_{combined}$.}
\end{tablenotes}
\end{table*}


The experimental results are shown in Table~\ref{tab:Performance of ownership verification}. Since there is no retraining conducted on the original DNN-watermarked, the suspect model (to-be-examined by HufuNet for ownership verification) demonstrates the same accuracy as that of our original model. Similarly, $EPH_{retrieved}$ is exactly the same as original EPH, so the accuracy of $HufuNet_{combined}$ equals to that of the original HufuNet. Therefore, the rebuilt $HufuNet_{combined}$ can always verify the ownership on the suspect model accurately considering not any kind of retraining on the stolen model is conducted\footnote{We also evaluate the integrity of HufuNet in Section \ref{subsec:integrity}, that is, without EPH, we will not claim ownership against innocent models.}.
According to Section \ref{subsec:Ownership Verification}, with $Acc_{ori}$ as 92.32\% and $\tau_{acc}$ as 15\%, the accuracy of $HufuNet_{combined}$ above 80\% means successful ownership verification. In the following experiments, we will just show HufuNet (combined) accuracy to indicate ownership verification.

%--------------------------------------------------------------------------%

\begin{table}
\centering
\footnotesize
\caption{Robustness against Kernels Cutoff}
\label{tab:robustnesscuttingoffkernels}
\begin{tabular}{m{1.17cm}
<{\centering}|m{1.5cm}
<{\centering}|m{2.5cm}
<{\centering}|m{1.2cm}
<{\centering}}
\hline
\textbf{DNN}&\textbf{Variance}& \textbf{Accuracy of DNN-watermarked}&\textbf{HufuNet Accuracy} \\
\hline \hline
\multirow{3}{*}{\text{VGG11}}&\text{Original}&\text{77.77$\%$}&\text{92.32$\%$} \\
\text{}&\text{Cut off}&\text{72.70$\%$}& \text{-} \\
\text{}&\text{Restore}&\text{72.70$\%$}& \text{92.14$\%$}\\ \hline


\multirow{3}{*}{\text{Resnet18}}&\text{Original}&\text{86.14$\%$}& \text{92.32$\%$} \\
\text{}&\text{Cut off}&\text{80.28$\%$}& \text{-} \\
\text{}&\text{Restore}&\text{80.28$\%$}& \text{92.38$\%$}\\ \hline


\multirow{3}{*}{\text{GoogLeNet}}&\text{Original}&\text{90.85$\%$}& \text{92.32$\%$} \\
\text{}&\text{Cut off}&\text{85.10$\%$}& \text{-} \\
\text{}&\text{Restore}&\text{85.10$\%$}& \text{92.02$\%$}\\ \hline

\end{tabular}
\end{table}

\vspace{-4pt}
\subsection{Robustness} 
\label{subsec:Robustness}
Due to the stealthiness of EPH (as shown in Section \ref{exp_stealthiness}), a targeted destruction (knowing where EPH is and destructing it correspondingly) is almost impossible. The adversary certainly can initialize and retrain all the convolutional layers of the stolen model. In this scenarios however, the adversary would rather train his/her own model than stealing $f_{wm}$, since those two procedures demand similar amount of computing resources and training data. In contrast, adversaries would prefer ``blindly'' revising the model, e.g., fine-tuning, pruning, kernels cutoff/supplement, etc., hoping to destruct embedded watermarks. 
%Even if adversaries perform such model change operations significantly on watermarked models, it is desired that the embedded watermarks can be still detected from the changed models. 

\noindent\textbf{Robustness against fine-tuning.}
\label{finetunig}
%With a small dataset available, fine-tuning DNN models is a frequently-used approach that can be leveraged by adversaries to retrain the stolen model, hoping to destruct any watermark embedded inside. 
We trained five models in total (with our watermark EPH embedded): VGG11, GoogLeNet, Resnet18 on CIFAR-10, Resnet34 on CIFAR-100, and LSTM on IMDB. We assume adversaries only have access to the testing dataset (provided by the model owner to test the performance of the model, including 10,000 samples), and try to leverage it to fine-tune the stolen model. Referring to the settings in \cite{li2019prove}, adversaries divide their available dataset into two parts, 80\% as the training dataset and 20\% as testing dataset. Same as \cite{adi2018turning}, we also set initial learning rate $\lambda=0.001$ and the delay factor as 0.0005 to fine-tune DNNs-watermarked using SGD (Stochastic Gradient Descent). The maximum number of epochs for fine-tuning is set as 100 according to \cite{li2019prove}, and the incremental step of the epoch is set as 10. As $\lambda$ decreases to a very small number, the parameters of DNNs-watermarked will rarely change, which indicates the model tends to be stable during fine-tuning. As shown in Table~\ref{tab:Robustness against Finetuning}, regarding the DNNs-watermarked, their accuracy drops at different scale when fine-tuned up to 40 epochs. As the number of epochs keeps increasing, the accuracy either gets improved or becomes stable. In contrast, the accuracy of $HufuNet_{combined}$ tends to be very stable, always above 90\%, which suffices ownership verification (above 80\%). Therefore, the fine-tuning process does not affect our EPH.

\noindent\textbf{Robustness against pruning.} 
%Generally, the goal of model pruning is to cut off redundant parameters, but still try to maintain similar performance as the original DNN model. Hence, adversaries can leverage model pruning approach, hoping to destruct any watermark embedded inside. After stealing a DNN model, the adversaries would like to prune it without retraining it or losing its performance too much. Hence, they prefer to prune less important parameters, e.g., those with smaller absolute values, since such parameters are believed to have little impact on the performance of DNN models. 
To evaluate the robustness of HufuNet against pruning, we first embed our watermark EPH into VGG11, GoogLeNet, Resnet18, Resnet34 and LSTM, and then prune 10\% to 90\% parameters of each model based on their absolute values respectively. We adopt the commonly used pruning technique in ~\cite{han2015learning}, which eliminates the parameters with smaller absolute values, thus believed to have little impact on the performance of the models. We choose such model pruning approach, which is consistent with our assumption of the adversaries' capability, i.e., lack of sufficient training dataset and/or computing resources. Table~\ref{Robustness against Pruning} shows the experimental results on the accuracy of the corresponding DNNs-watermarked and HufuNet after pruning. Based on the results, we find that even if the DNNs-watermarked have been pruned to be considered as ``fail'' on the main task (e.g., the accuracy of VGG11, GoogLeNet, Resnet18, Resnet34 has been reduced to 50.74\%, 10.00\%, 10.00\% and 1.10\%, respectively) after 80\% pruning, the accuracy of $HufuNet_{combined}$ is still above 80\%, satisfying the preset threshold $\tau_{acc}$. For 90\% pruning, the accuracy of $HufuNet_{combined}$ drops below 80\%, but this high degree of pruning almost completely ruin the main task of the model. It is interesting that the accuracy of LSTM does not drop as significantly as other models, probably due to its larger parameter redundancy when dealing with simple tasks. Overall, the high accuracy of $HufuNet_{combined}$ upon heavy pruning indicates it is highly robust against pruning.

\noindent\textbf{Robustness against kernels cutoff/supplement.}
%Owing to there is no need of training resource and training dataset for adversary about cutting off kernels attack, attacker can change the number of total kernels: N. However the verification ownership of HufuNet depends on N. N changed will make our HufuNet failed to verify ownership.}
We evaluate the robustness of HufuNet against kernels cutoff attack on VGG11, Resnet18, and GoogLeNet. Resnet34 and LSTM are not evaluated, since the structure of the former is similar as Resnet18 and the latter is innately immune from such attack (as discussed in Section \ref{subsec:threat}). Since the removal of the convolution kernels will reduce the performance of $f_{cutoff}$, we control the kernels cutoff rate as 6.75\%, 2.30\% and 4.77\% respectively for the above three models, to ensure their accuracy does not drop significantly (around 5\%), i.e., 5.07\%, 5.86\% and 5.75\% respectively. Then we use the above proposed cosine similarity approach to restore the structure of $f_{cutoff}$ and supplement 0 for the missing kernels (cut off). As shown in Table \ref{tab:robustnesscuttingoffkernels}, the accuracy of HufuNet is 92.14\%, 92.38\%, and 92.02\% for the three models respectively, which are sufficient to verify the ownership (above 80\%). The evaluation result of kernels supplement is quite similar to that of kernels cutoff, since both the structure and the number of kernels are changed in a similar way. 
%Due to page limit, we just show the results of kernels cutoff.

\noindent\textbf{Analysis of Robustness.} Due to the stealthiness (evaluated in Section \ref{exp_stealthiness}) and small scale of EPH in DNN-watermarked (EPH consumes 1.48\%$\sim$3.44\% of the parameter space of CNN models, and 13.38\% of the parameter space of the LSTM model, based on our experiment in Section \ref{subsec:Performance}), it is difficult for model pruning and fine-tuning to destroy the embedded watermark. The robustness of EPH against pruning and fine-tuning is also attributed to the parameter redundancy in DNN models. Usually a portion of parameters (e.g., the top 50\% parameters with large absolute values) contributes most to the task of a DNN model, while the other parameters can be considered ``redundant'' in the parameter space, making minor contribution to the model's task. Model retraining mainly affects those not-so-important values in the parameter space of DNN-watermarked; otherwise, the performance of the retrained model would be significantly worse than the watermarked model, which defeats the purpose of ownership verification. As long as a majority of significant parameters in EPH remains stable in model retraining, ownership verification can be performed robustly.


%\noindent\textbf{Robustness against initializing one layer.} More experienced adversaries may randomly choose one layer from their stolen model, initialize its parameters, and retrain it to ruin any watermark embedded. This is a stronger threat model compared with fine-tuning or pruning discussed above, especially for those approaches that embed watermark into one or several layers, since the probability that the adversaries happen to initialize the layers with watermark embedded is not negligible. Our HufuNet should survive from such elimination, sine the EPH is distributed across all layers of the DNN-watermarked, rather than on one or several layers. \lpz{We simulate such attack by initializing each layer of the convolutional layers of Resnet18. Then we freeze the parameters in the other layers, and fine-tune these initialized layers. And we also use 80\% of test dataset as training dataset and 20\% as testing dataset, and set the epochs of fine-tuning as 100.} \shengzhi{Where is the data?}

\ignore{
\begin{table}
\centering
\footnotesize
\caption{Initialize one layer of Resnet18}
\label{tab:Initialize_one_layer_of_Resnet18}
\begin{tabular}{m{1.3cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1.2cm}
<{\centering}|m{1.4cm}
<{\centering}|m{1.2cm}
<{\centering}}
\hline
\textbf{layers}& \textbf{EPH}& \textbf{Resnet18}& \textbf{Occupation}& \textbf{Accuracy}\\
\hline \hline
\textbf{conv1}& \text{0}& \text{1728}& \text{0$\%$}& \text{92.32$\%$}\\ \hline
\textbf{conv2} & \text{1125}& \text{36864}& \text{3.05}& \text{92.30$\%$}\\ \hline
\textbf{conv3}& \text{1008} &\text{36864}& \text{2.73$\%$}& \text{92.26$\%$} \\ \hline
\textbf{conv4}& \text{981} &\text{36864}& \text{2.66$\%$}& \text{92.30$\%$} \\ \hline
\textbf{conv5}& \text{945} &\text{36864}& \text{2.56$\%$}& \text{92.21$\%$} \\ \hline
\textbf{conv6}& \text{2304} &\text{73728}& \text{3.12$\%$}& \text{92.27$\%$} \\ \hline
\textbf{conv7}& \text{4050} &\text{147456}& \text{2.75$\%$}& \text{91.81$\%$} \\ \hline
\textbf{conv8}& \text{216} &\text{8192}& \text{2.64$\%$}& \text{91.75$\%$} \\ \hline
\textbf{conv9}& \text{4806} &\text{147456}& \text{3.26$\%$}& \text{91.68$\%$} \\ \hline
\textbf{conv10}& \text{4329} &\text{147456}& \text{2.94$\%$}& \text{91.40$\%$} \\ \hline
\textbf{conv11}& \text{8388} &\text{294912}& \text{2.84$\%$}& \text{90.99$\%$} \\ \hline
\textbf{conv12}& \text{17253} &\text{589824}& \text{2.84$\%$}& \text{90.99$\%$} \\ \hline
\textbf{conv13}& \text{1080} &\text{32768}& \text{3.30$\%$}& \text{89.73$\%$} \\ \hline
\textbf{conv14}& \text{16182} &\text{589824}& \text{2.74$\%$}& \text{87.94$\%$} \\ \hline
\textbf{conv15}& \text{16137} &\text{589824}& \text{2.74$\%$}& \text{84.39$\%$} \\ \hline
\textbf{conv16}& \text{33246} &\text{1179648}& \text{2.82$\%$}& \text{71.31$\%$} \\ \hline
\textbf{conv17}& \text{65646} &\text{2359296}& \text{2.78$\%$}& \text{25.48$\%$} \\ \hline
\textbf{conv18}& \text{3726} &\text{131072}& \text{2.84$\%$}& \text{25.33$\%$} \\ \hline
\textbf{conv19}& \text{66573} &\text{2359296}& \text{2.82$\%$}& \text{10.94$\%$} \\ \hline
\textbf{conv20}& \text{66195} &\text{2359296}& \text{2.81$\%$}& \text{10.01$\%$} \\ \hline
\end{tabular}
\end{table}
}

\vspace{-4pt}
\subsection{Adaptiveness}
\label{subsec:adaptiveness}
Since HufuNet is essentially a parameter-level watermark, we must ensure the embedded watermark can still be correctly retrieved to verify ownership. We further evaluate it against functionality-equivalent attack in terms of structure adjustment and parameter adjustment on three neural network models: VGG11, Resnet18, and GoogLeNet. We choose not to evaluate Resnet34 and LSTM, since the structure of the former is similar to Resnet18 and the latter is a RNN with sigmoid as activation function (which is not subject to functionality-equivalent attack).

\noindent\textbf{Adaptiveness against Structure Adjustment.}
%Generally, the goal of structure adjustment is to obtain a functionality-equivalent model by adjusting the order of the input channels and the output channels of the stolen model without retraining it. In this way, the parameters of the stolen model can be shuffled to evade the detection of parameter-level watermark. 
To simulate the maximum capability of attackers, we shuffle the order of all convolution kernels of each layer, and at the same time we adjust the order of the inner layers of the convolution kernels to ensure functionality-equivalent. If there is a BatchNorm layer connected after a convolution layer, we also change its mean and variance according to the order of the corresponding convolution kernels. We use the approach discussed in Section \ref{subsec:restore} to restore the order of kernels. The experimental results are shown in Table \ref{tab:structureequivalent}. After reordering the convolution kernels of the DNNs-watermarked, the accuracy of VGG11, Resnet18 and GoogLeNet remains the same (functionally equivalent), but the accuracy of the combined HufuNet (without restore) decreases significantly from $92.32\%$ to $18.15\%$, $13.71\%$ and $8.22\%$ respectively. After restoring however, the accuracy of the combined HufuNet resumes to $92.32\%$, the same as the original HufuNet, thus allowing correct ownership verification. 

\noindent\textbf{Adaptiveness against Parameter Adjustment.} We also evaluate HufuNet against functionality-equivalent attack through parameter adjustment. 
%Particularly, such attack can be applied to DNN-watermarked with activation functions like ReLU, rather than Sigmoid. Hence, LSTM is not evaluated, since its internal activation function is Sigmoid. In our evaluation, 
We change the parameter values of each layer by multiplying these parameters by $c = 2^n$ (n is a randomly-choose integer for each layer ranging from -18 to 18), while still maintaining the functionality-equivalent of the overall model. We use the approach as discussed in Section \ref{subsec:restore} to restore the parameter values. The experiment result are shown in Table \ref{tab:parameterequivalent}. After adjusting parameters of the DNNs-watermarked (PMCG, i.e., parameter change), the accuracy of VGG11, Resnet18 and GoogLeNet remains the same (functionally equivalent), but the accuracy of the combined HufuNet (without restore) decreases significantly to $14.68\%$, $15.79\%$ and $25.52\%$ respectively. After restore however, the accuracy of the combined HufuNet resumes to $92.32\%$, the same as the original HufuNet, thus allowing ownership verification. 

\noindent\textbf{Adaptiveness against Channel Expansion.} \label{evaluation_channel_expansion} %\shengzhi{Where do you use this kind of label? Does it work as expected?}
We also evaluate HufuNet against channel expansion on VGG11. We randomly choose two adjacent layers (the fourth and fifth layers), and double the output dimension of the fifth layer and input dimension of the sixth layer by supplementing output/input channels (details in Appendix \ref{analysis_of_channel_expansion_principle}).
%\shengzhi{Pay attention here to see how subsection in Appendix is used. Check the entire paper.} 
Finally, we launch the structure adjustment attack to make it more difficult to trace the EPH. We use the approach discussed in Section \ref{subsec:restore} to restore EPH. After channel expansion and structure adjustment, the accuracy of VGG11 remains the same (functionally equivalent), but the accuracy of the combined HufuNet (without restore) drops to 9.91\%. After restore however, the accuracy of the combined HufuNet resumes to $92.32\%$, the same as the original HufuNet, thus allowing ownership verification.

\begin{table}
\centering
\footnotesize
\caption{Adaptiveness against Structure Adjustment}
\label{tab:structureequivalent}
\begin{tabular}{m{1.17cm}
<{\centering}|m{1.5cm}
<{\centering}|m{2.5cm}
<{\centering}|m{1.2cm}
<{\centering}}
\hline
\textbf{DNN}&\textbf{Variance}& \textbf{Accuracy of DNN-watermarked}&\textbf{HufuNet Accuracy} \\
\hline \hline
\multirow{3}{*}{\text{VGG11}}&\text{Original}&\text{77.77$\%$}&\text{92.32$\%$} \\
\text{}&\text{Reorder}&\text{77.77$\%$}& \text{18.15$\%$} \\
\text{}&\text{Restore}&\text{77.77$\%$}& \text{92.32$\%$} \\ \hline


\multirow{3}{*}{\text{Resnet18}}&\text{Original}&\text{86.14$\%$}& \text{92.32$\%$} \\
\text{}&\text{Reorder}&\text{86.14$\%$}& \text{13.71$\%$} \\
\text{}&\text{Restore}&\text{86.14$\%$}&  \text{92.32$\%$} \\  \hline


\multirow{3}{*}{\text{GoogLeNet}}&\text{Original}&\text{90.85$\%$}& \text{92.32$\%$} \\
\text{}&\text{Reorder}&\text{90.85$\%$}& \text{8.22$\%$} \\
\text{}&\text{Restore}&\text{90.85$\%$}& \text{92.32$\%$} \\ \hline

\end{tabular}
\end{table}


\begin{table}
\centering
\footnotesize
\caption{Adaptiveness against Parameter Adjustment}
\label{tab:parameterequivalent}
\begin{tabular}{m{1.17cm}
<{\centering}|m{1.5cm}
<{\centering}|m{2.5cm}
<{\centering}|m{1.2cm}
<{\centering}}
\hline
\textbf{DNN}&\textbf{Variance}& \textbf{Accuracy of DNN-watermarked}&\textbf{HufuNet Accuracy} \\
\hline \hline
\multirow{3}{*}{\text{VGG11}}&\text{Original}&\text{77.77$\%$}&\text{92.32$\%$} \\
\text{}&\text{PMCG}&\text{77.77$\%$}& \text{22.29$\%$} \\
\text{}&\text{Restore}&\text{77.77$\%$}& \text{92.32$\%$} \\ \hline
\multirow{3}{*}{\text{Resnet18}}&\text{Original}&\text{86.14$\%$}&\text{92.32$\%$} \\
\text{}&\text{PMCG}&\text{86.14$\%$}& \text{14.68$\%$} \\
\text{}&\text{Restore}&\text{86.14$\%$}& \text{92.32$\%$} \\ \hline
\multirow{3}{*}{\text{GoogLeNet}}&\text{Original}&\text{90.85$\%$}&\text{92.32$\%$} \\
\text{}&\text{PMCG}&\text{90.85$\%$}& \text{25.52$\%$} \\
\text{}&\text{Restore}&\text{90.85$\%$}& \text{92.32$\%$} \\ \hline
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[1] PMCG refers to the DNN-watermarked whose parameters have been adjusted to launch functionality-equivalent attack. 
%Restore indicates the to-be-protected DNN has restored from parameter equivalent attack. Difference indicates the parameter difference our local HufuNet and extracted HufuNet from to-be-protected DNN.
\end{tablenotes}
\end{table}






%--------------------------------------------------------------------------%
%--------------------------------------------------------------------------%

\subsection{Against Synthetic Attacks}
\label{subsec:combination adaptiveness with robustness}
After stealing a DNN model, the adversaries may try their best to undermine any watermarks embedded inside, e.g., utilizing fine-tuning, pruning, functionality-equivalent attack (structure/parameter adjustment and channel expansion). Below, we synthesized an advanced attack by combining the above attack methods to simulate the adversaries' best effort, and evaluate HufuNet against such a synthetic attack. First, we randomly choose two adjacent layers (4th, and 5th in our experiment) of VGG11 (with our watermark EPH embedded) to launch the channel expansion attack. Then, we fine-tune VGG11 as we did in Section \ref{finetunig} using the test dataset in 100 epochs. Afterward, we randomly select six layers to launch the functionality-equivalent attack. The structure adjustment is applied to two layers. The parameter adjustment is applied to another two layers, and both structure adjustment and parameter adjustment are applied to the other two layers. In the end, we prune it with the pruning rate of 10\%. For watermark detection, we retrieve $EPH_{retrieved}$ from the attacked model at its original embedding locations and merge $EPH_{retrieved}$ with our local SPH to obtain $Hufu_{combined}$. 

As shown in Table \ref{tab:advancedattack}, at the pruning rate of 10\%, the accuracy of $HufuNet_{combined}$ without restoring (``Direct'' in the table) drops to 10.23\%. After utilizing the restore approach in Section \ref{subsec:restore}, the accuracy of $Hufu_{combined}$ increases to 90.74\% with 100\% parameters correctly restored, thus allowing ownership verification. We also evaluate our restore approach against heavy pruning over the stolen model, up to 50\%. With the pruning rate of 30\%, HufuNet accuracy after restore is 83.95\%, still above the threshold for ownership verification (80\%), with 96.73\% of all embedded kernels correctly restored. The reasons that the restore rate is still above 96\% even at the pruning rate of 30\% are twofold. On the one hand, larger-value parameters contribute significantly to both the cosine similarity and SVD, while pruning starts to zeorize smaller-value parameters with larger-value ones unchanged. On the other hand, the cosine similarity and SVD compare the stolen model and the watermarked model at the granularity of channels, each of which includes a large number of parameters, i.e., $64*3*3$. Even at pruning rate of 30\%, there still exist lots of parameters (almost half on average) unchanged in most of the channels, resulting in higher cosine similarity and SVD values based on our experiments. At the pruning rate of 40\% however, the accuracy of HufuNet after restore is 51.25\% (below the threshold of 80\%), but the accuracy of the stolen VGG11 drops to 43.30\%, making it almost useless in performing its original task. Overall, based on the evaluation results, synthetic attacks launched by more capable adversaries can still be caught by our HufuNet watermark with the pruning rate up to 30\%. As the pruning rate keeps increasing, i.e., above 40\%, HufuNet fails ownership verification, but the adversaries end up with an almost useless stolen model (accuracy below 45\%).

\begin{table}
\begin{threeparttable}
\centering
\footnotesize
\caption{Against Synthetic Attacks}
\label{tab:advancedattack}
\begin{tabular}{m{1.5cm}
<{\centering}|m{1cm}
<{\centering}|m{1.1cm}
<{\centering}|m{1.1cm}
<{\centering}|m{1.9cm}
<{\centering}}
\hline

\multirow{2}{*}{\textbf{Pruning Rate}}&\multirow{2}{*}{\textbf{VGG11}}&\multicolumn{2}{c|}{\textbf{HufuNet Accuracy}}&\multirow{2}{*}{\textbf{Restored Rate}}\\
\cline{3-4}

\textbf{}& \textbf{}& \textbf{Direct}& \textbf{Restored}& \textbf{}\\
\hline \hline
\textbf{10\%}& \text{73.85\%}& \text{10.23\%}& \text{90.74\%}& \text{100.00\%}\\
\hline
\textbf{20\%}& \text{73.85\%}& \text{11.13\%}& \text{88.08\%}& \text{99.85\%}\\
\hline
\textbf{30\%}& \text{73.80\%}& \text{8.87\%}& \text{83.95\%}& \text{96.73\%}\\
\hline
\textbf{40\%}& \text{43.30\%}& \text{10.56\%}& \text{51.25\%}& \text{88.82\%}\\
\hline
\textbf{50\%}& \text{9.20\%}& \text{10.14\%}& \text{10.17\%}& \text{75.15\%}\\
\hline
%\textbf{60\%}& \text{8.90\%}& \text{10.53\%}& \text{37.94\%}& \text{97.60\%}\\ \hline
\end{tabular}
\end{threeparttable}
\vspace{-7mm}
\end{table}

%\lpz{The adversaries can also try to undermine any watermarks by kernels cutoff/supplement and fine-tuning. The adversaries choose two adjacent layers of stolen model with matrices A and B, then double the output dimension of $A$ by kernels supplement, and double the input dimension of $B$ accordingly. These two expanded matrices are defined as $A'$ and $B'$, which have the property that $(A' B') x = (A B) x$. $x$ is the feature map propagated in neural networks. In this process, the adversaries only need to add some parameters through mathematical deduction, and there is no training process. Then, they fine-tune the resulting model slightly to perturb the weights. The embedded watermark may be destroyed because each parameters has been split between $A'$ and $B'$.}

\subsection{Stealthiness}
\label{exp_stealthiness}
%Given a stolen DNN model, the adversaries may examine the model, either by investigating its structure and parameters, or by observing its outputs from particular inputs, to determine whether or not any watermark exists in the model. 
According to the results in Section \ref{subsec:Performance}, our watermark EPH only occupies a small portion of the DNNs-watermarked, thus difficult to be noticed. Although there exists a correlation (i.e., HMAC) between the embedding location in DNN-watermarked and the kernel parameters plus their indices in HufuNet, the strength of the key used to compute the HMAC and the secrecy of the indices in HufuNet make learning such correlation computationally hard. Hence, it is difficult for adversaries to learn the existence of the embedded watermark. Instead, they may resort to a statistical approach, e.g., examining the distribution of parameter values or their gradients of correct labels for any embedded watermark's footprint.  


\begin{comment}
\begin{figure*}[h]
\centering
\subfigure[]
{
\begin{minipage}[t]{0.5\textwidth}
\centering
%\includegraphics[width=0.95\textwidth]{fig/bothparameter.jpg}
\epsfig{figure=fig/bothparameter.jpg, width=0.95\textwidth} 
%\caption{fig2}
\end{minipage}
}

\subfigure{
\begin{minipage}[t]{0.5\textwidth}
\centering
%\includegraphics[width=0.95\textwidth]{fig/bothparameter.jpg}
\epsfig{figure=fig/bothgradient.jpg, width=0.95\textwidth} 
%\caption{fig2}
\end{minipage}
}%

\caption{Distribution of Parameter Values and Distribution of Gradients of Parameter Values}
\label{fig:Distribution}
\end{figure*}
\end{comment}


The adversaries with expertise in deep learning may have sufficient knowledge and understanding of their stolen model, e.g., roughly how the parameter values distribute. Therefore, we measure whether our watermark EPH will change the distribution of the parameter values in DNN-watermarked. We find that the distribution of the parameter distribution of DNN-to-be-protected (without EPH) and DNN-watermarked (with EPH) is too close to be distinguished, as shown in Figure \ref{fig:Distribution}(a) in Appendix. In addition, Grad-CAM~\cite{selvaraju2017grad} finds that the gradients of the score of true labels flowing back are global-average-pooled to obtain the neuron importance weights. The experienced adversaries are very likely to analyze the gradient distribution of neurons to discover any embedded watermark. Therefore, we choose 8,000 input images in the CIFAR-10 testing dataset, and for each correct label, compute the gradient of EPH and other parameters in DNN-watermarked. We find their distribution closely resembles each other, thus hard for adversaries to learn any embedded watermark evidence. The gradient distribution of EPH and other parameters in DNN-watermarked are compared in Figure \ref{fig:Distribution}~(b) in Appendix. 

%Since the embedding approach, i.e., Algorithm \ref{alg:Position-injected}, is public, the adversaries are aware that if a kernel in the stolen model belongs to the embedded watermark, its index in the stolen model (i.e., embedding position) should be derived from Line 3 in Algorithm \ref{alg:Position-injected}. Since HMAC and XORPMV are also public, to determine whether or not a particular kernel in the stolen model comes from HufuNet, the adversaries can launch brute force attack by searching all possible keys and its original index in HufuNet ($i$, up to XXX, the total number of kernels in our HufuNet), with the knowledge of its parameter values and its index (i.e., its current position) in the stolen model, and the number of all kernels in the stolen model ($N$). We find that such brute force attack is computationally hard based on our evaluation. We embedded our watermark (XXX kernels) into VGG11 with 1,024,192 kernels in total. It takes about XXX seconds to compute one HMAC operation (i.e., SHA256 in our experiment) using our server with Intel Xeon E5-2620 v4@2.10GHz CPU. In the worst case, the adversaries need XXX seconds to traverse the key space (According to~\cite{microsha256}, the recommended size of key for SHA256 is 64 bytes) and all possible $i$ (up to XXX) for one kernel in VGG11. \shengzhi{replace XXX in this paragraph}




%--------------------------------------------------------------------------%
%--------------------------------------------------------------------------%

%\vspace{-11pt}
\subsection{Security}
\label{subsec:security1}
%Knowing our watermarking approaches, the adversaries may forge their own watermarks for the DNN models they steal, and claim their ownership fraudulently (also called ambiguity attack~\cite{fan2019rethinking}).

An intuitive idea is that the adversary forges a valid HufuNet-style watermark from the public dataset $D_s$ and embeds it into DNN-watermarked. In particular, the adversary first trains a HufuNet from $D_s$; he/she then chooses a secret key and embeds EPH from the forged HufuNet into DNN-watermarked following the watermark embedding algorithm. In case of ownership dispute, the adversary may perform ownership verification on his/her stolen model, from which the forged watermark can be detected following the ownership verification algorithm. In such a case, the adversary's secret key would be different from the owner's secret key with an overwhelming probability. Therefore, it is highly unlikely that the adversary's forged watermark overwrites the owner's watermark in DNN-watermarked. Consequently, the adversary can only present a model with both his/her watermark and the owner's watermark detected, while the owner of the model can present the original DNN-watermarked with only the owner's watermark detected. It is thus clear who is the true owner to resolve the dispute.

Therefore, the adversary has to leverage existing parameters in the stolen model rather than revising any. Meanwhile, two requirements have to be satisfied to forge a valid and effective HufuNet-style watermark: (R1) the accuracy of the forged HufuNet passes the threshold; (R2) the positions where the embedded kernels (EPH) are retrieved should satisfy the correlation based on Line 3 in Algorithm \ref{alg:Position-injected}. Below we discuss and evaluate two different watermark forging attacks depending on which requirement to satisfy first: the first accuracy then correlation and first correlation then accuracy.

%According to Section \ref{subsec:justification}, forging a new HufuNet based on the public training dataset and embedding the corresponding EPH into the stolen model will bring the adversaries into a situation that they can only present a model that is embedded with both their watermark and the owner's watermark, while the owner can present the original DNN-watermarked with the owner's watermark only. Therefore, the adversaries have to leverage the existing parameters in the stolen model, rather than revising any. Below, we evaluate the two watermark forging attacks discussed in Section \ref{subsec:justification}.


\noindent\textbf{First accuracy then correlation}
The adversary first trains his/her own HufuNet by designing a simple network structure and using the public training dataset. Once thoroughly tested, the adversary also divides it into two pieces and keeps the right piece as his/her SPH. Instead of embedding the left piece, the adversary searches the stolen model's parameter space for each of the convolution kernel of his/her EPH. An exact match of all the $3*3$ values of a kernel is hard to be found in general, so the adversary searches for closely-matched values, e.g., within the range of 25\% less and 25\% more of the searched value, which may still function similarly in the neural network. With those values found and retrieved (if lucky enough), the adversary can rebuild a $HufuNet_{combined}$ by combining them with the local SPH, and test its accuracy on the public training dataset. Note that the high accuracy of $HufuNet_{combined}$ is not enough. The adversary also needs to build the correlation between the embedding location and the parameter values of the kernel plus its original index in their HufuNet based on an appropriate key, according to Line 3 in Algorithm \ref{alg:Position-injected}.

%In particular, the adversary needs to find a key and a HMAC function, so that they can satisfy such correlation for all the found kernels from the stolen model. For each kernel found with close-enough values in the stolen model, the adversary needs to compute the hash based on the values, their original index in their HufuNet, and perform the modulo operation over the number of the parameters in the stolen model. The result needs to be exactly the index where the kernel is extracted from the stolen model. 

We simulate the attack in two steps. In the first step, we train a HufuNet and check whether we can find a closely-matched kernel in DNN-watermarked (VGG11, Resnet18 and GoogLeNet) for each kernel in EPH, by setting the range as between below n\% and above n\% of the searched values\footnote{Based on our experience, a larger range makes it easy to find matched kernels, but cannot guarantee the high accuracy of $HufuNet_{combined}$, thus failing the ownership claim.}. However, even when n\% is set to be large, e.g., 200\%, the small values (e.g., 10e-7) in kernels are still difficult to be matched. Therefore, we ignore those small values when we perform kernel matches, since they generally contribute very little to the classification task of DNN models. The threshold to filter out the small values is chosen by setting the pruning rate to be 10\%, because the accuracy of HufuNet decreases significantly at a larger pruning rate. As shown in Table \ref{tab:securityofhufunet}, when we set the range n\% to be 25\%, lots of kernels in EPH cannot find matches in DNN-watermarked, i.e., total 64.90\%, 47.86\%, 52.92\% found in VGG11, GoogLeNet, and Resnet18, respectively. Until we increase the range to 75\%, 90\%, and 110\% for VGG11, GoogLeNet, and Resnet18 respectively, all the kernels of EPH can be matched. However, the accuracy of such $HufuNet_{combined}$ is quite low, i.e., 53.74\%, 60.96\%, and 34.00\% respectively, failing the adversary's goal of forging a valid watermark. In the second step, we show the computational difficulty for even a determined adversary to build the correlation for the closely-matched kernels by traversing all possible keys for HMAC function. It takes about $2.18*10^{-4}$ seconds to compute one HMAC operation (i.e., SHA256 in our experiment) using our server with Intel Xeon E5-2620 v4@2.10GHz CPU. According to~\cite{microsha256}, the recommended size of key for SHA256 is 64 bytes, which results in $2^{512}$ different keys for SHA256. Therefore, it takes $2.18*10^{-4}*2^{512}$ seconds for the adversary to traverse all the keys to try the correlation for one kernel in the forged HufuNet, which is computationally hard. Note that such brute force cannot ensure an appropriate key can always be found to build the correlation for all the kernels (i.e., 27,952) in the forged HufuNet. 

\noindent\textbf{First correlation then accuracy.}
Since both the training dataset $D_s$ and the testing dataset $D_{s\_TEST}$ are standardized for training and verifying HufuNet (see Section \ref{subsec: watermark_Genaration}), the adversaries cannot forge a valid HufuNet with arbitrary datasets. However, it does not rule out the possibility of forging a valid HufuNet from the public dataset $D_s$ and $D_{s\_TEST}$ with high accuracy. It is possible that the parameter space of DNN-watermarked is large and includes sufficient values required by an adversary to match a forged HufuNet. However, to prevent the adversaries from associating the matched values between DNN-watermarked and a forged HufuNet, our embedding algorithm correlates each EPH kernel's embedding location in DNN-watermarked with a secret key, the parameter values of the EPH kernel, and its index through a secure HMAC function.  

Since Algorithm \ref{alg:Position-injected} is public, the adversary may randomly select a key, test each kernel in the stolen model based on Line 3 in Algorithm \ref{alg:Position-injected}, and try to find all the kernels that satisfy the correlation. The adversary can explore quite several different keys, e.g., 1,000, and check which key finds the most kernels that satisfy the correlation. If enough such kernels could be found based on a particular key, the adversary can claim those kernels are his/her EPH. To forge a valid HufuNet-style watermark, the adversary simply places those kernels into the convolution layers, randomly initializes a fully connected layer, and trains the fully connected layer using the public dataset $D_s$. Such watermark might have high accuracy on the public testing dataset as well. Although theoretically plausible, our experiment below shows that it is computationally tricky for the adversary to discover an appropriate secret key to find him/her enough kernels satisfying the correlation. 

We train VGG11 with our HufuNet watermark embedded, as DNN-watermarked. After stealing the model, the adversaries can try a random key on all the 1,024,192 kernels in VGG11, to find those kernels that satisfy the correlation as Line 3 in Algorithm \ref{alg:Position-injected}. We simulate this attack by testing 100 random keys, and find at most 3 kernels that can satisfy the desired correlation. With such a limited number of kernels, it is impossible to build convolutional layers of any DNN model. Brute force searching of all keys is computationally hard based on our evaluation. In the worst case, the adversary needs $2.18*10^{-4}*2^{512}$ seconds to traverse all the keys for just one kernel as presented above. Note that brute force searching of all possible keys may let the adversary obtain our key used to embed our HufuNet, but it is computationally hard to traverse all the keys (a key of 64 byte long means 2$^{256}$ different keys in total.).

%\lpz{The attack is extremely difficult, if not impossible, to locate a random key that can find enough kernels that satisfy the correlation to construct the convolution layers of a model based on our evaluation results as below. Note that brute force searching of all possible keys may let the adversary obtain our key used to embed our HufuNet, but it is computationally hard to traverse all the keys (a key of 64 byte long means 2$^{256}$ different keys in total.).}

%\lpz{We will show the computational difficulty for even a determined adversary to find watermarking kernels by traversing all possible keys of HMAC function. There are total 1,024,192 kernels in VGG11, but after HMAC operation on all kernels, only the HMAC value of 1.2 kernels matches their position successfully on average of 100 HMAC operation on 1,024,192 kernels. Meanwhile, the time to compute the hash (e.g., SHA256) of total 1,024,192 kernels in VGG11 with a specific key is 138.37 seconds using our computer with Intel Xeon E5-2620 v4@ 2.10GHz CPU and 2.23GB memory occupation in our experiment. Therefore, the total time for brute force attack will be $2^{512}*138.37$ seconds to find the appropriate kernels composing of convolution layers, which is computationally hard. So we also think this attack failed.}

%The time to compute the hash (e.g., SHA256) of total 27,952 convolution kernels in forged HufuNet with a specific key is \lpz{7.479 seconds} \lpz{on average of 1000 HMAC} using our computer with Intel Xeon E5-2620 v4 @ 2.10GHz CPU and 2.27GB \lpz{memory occupation} in our experiment. \shengzhi{replace XXX} According to~\cite{microsha256}, the recommended size of key for SHA256 is 64 bytes, which results in $2^{512}$ different keys for SHA256. Therefore, the total time for brute force attack will be \lpz{$2^{512}*7.479$} seconds, which is computationally hard. Note that such brute force attack cannot ensure an appropriate key can always be found to build the correlation.


\begin{table}
\begin{threeparttable}
\centering
\footnotesize
\caption{Security of $HufuNet$}
\label{tab:securityofhufunet}
\begin{tabular}{m{1.15cm}
<{\centering}|m{0.75cm}
<{\centering}|m{0.75cm}
<{\centering}|m{0.75cm}
<{\centering}|m{0.75cm}
<{\centering}|m{0.6cm}
<{\centering}|m{1cm}
<{\centering}}
\hline
\multirow{2}{*}{\textbf{Models}}&\multicolumn{5}{c|}{\textbf{Found Percentage at Different Thresholds}}&\multirow{2}{*}{\parbox{3cm}{\textbf{ HufuNet \\ Accuracy$^{1}$}}}\\
\cline{2-6}
\text{ }& \text{25\%}&\text{50\%}& \text{75\%}& \text{80\%}& \text{90\%} \\
\cline{2-7} \hline \hline
\textbf{VGG11}& \text{64.90$\%$}& \text{97.80$\%$} &\text{100$\%$}& \text{100$\%$}& \text{100$\%$}& \text{53.74$\%$} \\ \hline
\textbf{Resnet18}& \text{52.93$\%$}&  \text{93.24$\%$} &\text{99.99$\%$}& \text{100$\%$}& \text{100$\%$}& \text{34.00$\%$} \\ \hline
\textbf{GoogLeNet}& \text{47.86$\%$}& \text{87.76$\%$} &\text{99.84$\%$}& \text{99.97$\%$}& \text{100$\%$}& \text{60.96$\%$} \\ \hline
\end{tabular}
\begin{tablenotes}
\item[1] HufuNet Accuracy is measured when 100\% kernels are found at the lowest range for each model.
\end{tablenotes}
\end{threeparttable}
\end{table}

\begin{comment}
We simulate the above attack in two steps. In the first step, we train a HufuNet and check whether we can find a closely-matched kernel in DNN-watermarked (VGG11 and Resnet18) for each kernel in EPH, by setting the range as between below 100\% and above 100\%\footnote{Based on our experience, a larger range makes it easy to find matched kernels, but cannot guarantee high accuracy of $HufuNet_{combined}$, thus failing the ownership claim.}. \shengzhi{100\% seems too big.} As shown in Table \ref{tab:concealment}, XXX\% and XXX\% of kernels in EPH cannot find matches for VGG11 and Resnet18, respectively, causing low accuracy of $HufuNet_{combined}$. \shengzhi{replace XXX. In Table \ref{tab:concealment}, the same number of kernels for VGG11 and Resnet18? Why are there so may matches for VGG11?}
%Even if the adversary can find a close match for all kernels in $f_{wm}$, he/she needs to perform the second step in the attack, satisfying the hash-modulo correlation between the parameter values of the found kernel in $f_{wm}$, the index of the matched kernel in $f_{wm}$ and the position where the kernel is found in $f_{wm}$. 
In the second step, we show the computational difficulty for even a determined adversary to build the correlation for the matched kernels by traversing all possible keys. The time to compute the hash (e.g., SHA256) of the 27,952 (\shengzhi{which model}) convolution kernels with a specific key is 4 seconds \shengzhi{Better to use the number of instructions, since the time varies on different machines.}. According to ~\cite{microsha256}, the recommended size of key for SHA256 is 64 bytes. Therefore, the total time for brute force attack will be $2^{514}$s, \shengzhi{update it} which is computationally hard. \shengzhi{Find a source saying something like a powerful cluster of computers can run XXX instructions per second. So it will take XXX seconds for such a powerful cluster to finish this brute force attack.} Note that such brute force attack cannot ensure appropriate key can always be found to build the correlation. 
\end{comment}








\begin{comment}

\begin{table}
\begin{threeparttable}
\centering
\footnotesize
\caption{Security of $HufuNet$}
\label{tab:concealment}
\begin{tabular}{m{2.6cm}
<{\centering}|m{2cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1cm}
<{\centering}}
\hline
\textbf{DNN-watermarked (Range)}& \textbf{Not Find/Total$^{1}$}& \textbf{Percentage of Not Find}& \textbf{Accuracy$^{2}$}\\
\hline \hline
\textbf{VGG11(10\%)}& \text{$27952/27952$}& \text{100\%}& \text{$17.33\%$}\\
\hline
\textbf{Resnet18(10\%)}& \text{$27952/27952$}& \text{100\%}& \text{$10.64\%$}\\
\hline
\textbf{GoogLeNet(10\%)}& \text{$27952/27952$}& \text{100\%}& \text{$13.07\%$}\\
\hline
\textbf{VGG11(100\%)}& \text{$252/27952$}& \text{0.90\%}& \text{$53.36\%$}\\
\hline
\textbf{Resnet18(100\%)}& \text{$9463/27952$}& \text{33.85\%}& \text{$12.68\%$}\\
\hline
\textbf{GoogLeNet(100\%)}& \text{$3062/27952$}& \text{10.95\%}& \text{$68.08\%$}\\
\hline
\end{tabular}
\begin{tablenotes}
\item[1] Not Find/Total refers to the number of convolution kernels not found and the number of total kernels in DNN watermarked.
\item[2] Accuracy indicates the accuracy of the forged HufuNet, built based on the matched kernels.
\item[3] Range indicates the range of (Range)\% less and (Range)\% more of the searched value.
\end{tablenotes}
\end{threeparttable}
\end{table} 

\end{comment}



\begin{comment}
We mimic the adversary to perform the above attacks in two steps. In the first step, we train a HufuNet (HufuNet1 in Figure~\ref{tab:SecurityofHufu}) and check whether there are some kernels in DNN-watermarked (i.e., $f_{wm}$) matching the EPH of HufuNet1. Note that the perfect matching is almost impossible. So we assume to find a \textit{closely} match if the difference between a kernel in EPH and the kernel in HufuNet1 is less than a threshold (e.g., 0.1\% in our evaluation\footnote{A large threshold cannot guarantee a high accuracy of HufuNet and fail the ownership claim.}). Table~\ref{tab:SecurityofHufu} shows the percentage of kernels in EPH that have a closely matched kernel in $f_{wm}$. The number is XX\% for HufuNet1, which is quite low and hard to satisfy the ownership verification. We also repeat the process and train more HufuNets (HufuNet2$\sim$HufuNet10) with different initialization parameters; the results are similar. Even if the adversary can find suitable kernels, he needs to perform the second step in the attack: using the positions of the found kernels in $f_{wm}$ to reverse the key of a hash function, which is proved to be almost impossible~\cite{}. Thus, based on the evaluation, it is almost impossible for the adversary to claim the ownership of a DNN-watermarked.
\end{comment}


%\lpz{We simulate the above attacks by training 10 HufuNets with different initialization parameters, and limit parameters difference less than $10^{-5}$ to search for kernels with close-enough values in DNN-watermarked.  Table \ref{tab:SecurityofHufu} shows the percentage of kernels in EPH that have a closely matched kernel in DNN-watermarked and the $HufuNet_{combined}$ accuracy. In particular, for each convolution kernel of Forged HufuNets, we can locate a kernel with close-enough values in DNN-watermarked. With those kernels retrieved from DNN-watermarked and used as $EPH_{retrieved}$, we rebuild 100 different $HufuNet_{combined}$ for each forged HufuNet. Their accuracy on the testing dataset is 29.95\% on average, which is hard to satisfy the ownership verification. For the last step of correlation, on the above 10 forged HufuNet, we tried several different keys on five difference hash functions, MD5, SHA256, SHA512, SHA224, and non-keyed hash. None of them computes the correct correlation for even one kernel. In Table \ref{tab:SecurityofHufu}, we give the total execution time to compute the hash for one kernel, given a particular key. Considering the size of key used in the hash functions, it takes 17.82s for MD5, 19.87s for SHA256, 19.17s for SHA512, 21.24s for SHA224, 22.75s for non-keyed hash to try each possible key to test the correlation, which is computationally hard for the adversary. }

%\lpz{we define the time-consuming training as $T$. Then for each convolution kernel, they search for very-close values in the parameter space of DNN-watermarked, the time consuming of searching is defined as $S$. Once found, they use a hash to compute the location and examine if it matches the real location, the time consuming of each hash is $H$. Maybe they use different keys of hash to map, total $K$ key. The total time-consuming is $O(T+S+K*H)$. We analyze the parameters: $T, S, H$. In our setting, $T$ is 12 min 10s to train forged HufuNet; we use the dichotomy to search, and $S$ is 2min48s with 11164362 parameters to search. We evaluate the time of different hash way to inject, MD5 is 17.82s, SHA256 is 19.87s, SHA512 is 19.17s on average, SHA224 is 21.24s, and hash without the key is 22.75s. And we test these five hash per 200, and the result is shown as Table \ref{tab:Securitycasestudy}. It can be seen that even attackers forge HufuNet, they cannot forge a hash to correspond the position, so they unable to fraudulently claim ownership.}



\begin{comment}
\begin{table*}[h]
\begin{threeparttable}
\centering
\footnotesize
\caption{Simulate Attacker on Forged HufuNet}
\label{tab:forgedhufunet}
\begin{tabular}{m{5cm}
<{\centering}|m{2cm}
<{\centering}|m{2cm}
<{\centering}|m{2cm}
<{\centering}|m{2cm}
<{\centering}|m{2cm}
<{\centering}}
%\Xhline{3\arrayrulewidth}
\hline
\textbf{HufuNet Architecture}& \textbf{Front}& \textbf{Middle}& \textbf{Back}& \textbf{Middle\&Back}&\textbf{Global}\\ \hline \hline

\textbf{Same to our HufuNet}& \text{$59.53\%$}& \text{$10.00\%$}& \text{$10.00\%$}& \text{$10.00\%$}&\text{$10.00\%$}\\ \hline

\textbf{Not same to our HufuNet}& \text{$47.58\%$}& \text{$10.00\%$}& \text{$10.00\%$}& \text{$10.00\%$}&\text{$10.00\%$}\\ \hline
\end{tabular}
\begin{tablenotes}
\item[1]Same to our HufuNet indicates the forged HufuNet's architecture is same as real HufuNet; Front indicates the accuracy of forged HufuNet whose $Embedded\ Hufu$'s parameter are all coming from the front convolutional layers of DNN-watermarked.
\end{tablenotes}
\end{threeparttable}
\end{table*}
\end{comment}


%\lpz{Specifically, we simulate attackers trying to extract certain parameters in HMAC way from the middle and back part of DNN-watermarked as $Embedded\ Hufu$, further generate the corresponding HufuNet by forging the local $Verified\ Hufu$}, and thereby achieving fraudulent verification of DNN ownership of the target watermark. We conduct the simulation experiment on VGG11, GoogLeNet, Resnet18, Resnet34, and LSTM, each DNN with 10 random keys for HMAC function to choose positions for forging $Embedded Hufu$. Further, we calculate the average accuracy of these 10 forged HufuNet. \kai{it is better to evaluate on more models/datasets.}In order to make the experiment representative, we design 10 types of forged HufuNet, five of them have the same architecture as the real HufuNet, others have different architecture, which includes five convolutional layers with one fully connection layer. We randomly extract parameters from the front, middle, back, and global of Resnet18, and then embed the extracted parameters into the parameter space of the forged $Embedded\ Hufu$ architecture. Furthermore, we freeze the $Embedded\ Hufu$, only train $Verified\ Hufu$ on the training dataset of Fashion-MNIST in 100 epochs and get forged HufuNet, those forged HufuNet are tested on a test dataset of Fashion-MNIST. The average accuracy rate is shown in Table\ref{tab:forgedhufunet}, the accuracy of most forged HufuNet on the test dataset is 10\%, the best case is 59.53\%, which is still less than the threshold that can verify ownership of our DNN-watermarked. The experiment shows that it is too difficult for attackers to forge HufuNet to achieve fraudulent verification of the ownership of the DNN-watermarkeds.


%--------------------------------------------------------------------------%
%--------------------------------------------------------------------------%
\vspace{-10pt}
\subsection{Integrity}
\label{subsec:integrity}
%\lpz{When the watermark detection approach is applied to an innocent model, the result of ownership verification should be negative as required by watermark integrity, even if the innocent model highly resembles the owner's watermarked model in various ways, e.g., trained using similar network structure or dataset.} 
We evaluate the integrity of HufuNet by testing its ownership verification on innocent models not copied or retrained from ours. In this experiment, we intend to use the innocent models that always share the same network structure and the same task as ours, thus highly resembling our watermarked models. In particular, we consider two different kinds of such innocent models: (Innocent 1) the same training dataset as DNN-watermarked and (Innocent 2) a different training dataset than DNN-watermarked. We train each innocent model for 100 epochs, and each epoch begins with different initialization parameters to ensure high accuracy. We use the models obtained above as the innocent models, without embedding our watermark inside them. Upon ownership verification, we build $HufuNet_{combined}$ by combining the local SPH and the $EPH_{retrieved}$ from the innocent models based on the computed embedding locations. The experimental results are shown in Table \ref{tab:integrity}. The accuracy of $HufuNet_{combined}$ is 11.98\% for Innocent 1 and 9.97\% for Innocent 2 on average. Therefore, none of the innocent models can be falsely claimed as ours. For other models with different structures, main tasks, or training datasets, it is unlikely for HufuNet to claim ownership falsely.

\begin{table}
\begin{threeparttable}
\centering
\footnotesize
\caption{Integrity of HufuNet}
\label{tab:integrity}
\begin{tabular}{m{1.5cm}
<{\centering}|m{0.75cm}
<{\centering}|m{1.25cm}
<{\centering}|m{0.95cm}
<{\centering}|m{0.95cm}
<{\centering}|m{0.75cm}
<{\centering}}
\hline
\textbf{ }& \textbf{VGG11}& \textbf{GoogLeNet}& \textbf{Resnet18}& \textbf{Resnet34}& \textbf{LSTM}\\
\hline \hline
\textbf{Innocent 1$^{1}$}& \text{13.06$\%$} &\text{14.39$\%$}& \text{10.02$\%$}& \text{12.21$\%$}& \text{10.21$\%$} \\ \hline
\textbf{Innocent 2$^{2}$}& \text{10.59$\%$} &\text{10.00$\%$}& \text{9.27$\%$}& \text{10.00$\%$}& \text{9.99$\%$} \\ \hline
\end{tabular}
\begin{tablenotes}
\item[1] Innocent 1 refers to the innocent model with the same architecture and the same task trained with the same dataset as ours.
\item[2] Innocent 2 refers to the innocent model with the same architecture and the same task but trained with different dataset than ours.
\end{tablenotes}
\end{threeparttable}
\end{table}

%--------------------------------------------------------------------------%
%--------------------------------------------------------------------------%
\subsection{Fidelity}
\label{subsec:fidelity}
%\lpz{Watermark fidelity means that the performance of a watermarked model should be equivalent to the original model and that the impact of watermark embedding on the model's performance is negligible. Watermark fidelity is critical in certain DNN applications such as autonomous driving where even 1\% of performance loss is intolerable.}
Ideally, our watermark EPH should have a negligible impact on the performance of the DNN-to-be-protected. 
%In other words, trained on the same dataset, DNN-to-be-protected and DNN-watermarked should have similar accuracy on the main task. 
To demonstrate such fidelity, we perform experiments on the models trained on datasets as in Table \ref{tab:parameter} and evaluate the accuracy of DNNs-to-be-protected and DNNs-watermarked. Table~\ref{tab:fidelity} shows that the accuracy of DNNs-watermarked is always quite close to that of DNNs-to-be-protected. We believe it is mainly because our watermark EPH only occupies a small portion of the entire parameters of DNNs-watermarked and participates in the training of DNNs-watermarked, thus incurring little impact on their accuracy. 

%On the other hand, though only a small potion, our EPH is embedded before the training of DNN-watermarked, thus contributes to it by ``transfering'' some capabilities of feature extraction from EPH. Therefore, DNN-watermarked converges faster as discussed in Section \ref{subsec: watermark_Genaration}. \kai{do similar situations (i.e., increasing the accuracy) happen in other studies before? The two reasons look not so convincing.} \shengzhi{The two reasons look contradictory to each other: it is only a small portion, so with little impact on the accuracy of DNN-watermarked, but it improves its accuracy. }

\begin{table}
\begin{threeparttable}
\centering
\footnotesize
\caption{Fidelity of HufuNet}
\label{tab:fidelity}
\begin{tabular}{m{1.4cm}
<{\centering}|m{0.8cm}
<{\centering}|m{1.25cm}
<{\centering}|m{0.95cm}
<{\centering}|m{0.95cm}
<{\centering}|m{0.75cm}
<{\centering}}
\hline
\textbf{ }& \textbf{VGG11}& \textbf{GoogLeNet}& \textbf{Resnet18}& \textbf{Resnet34}& \textbf{LSTM}\\
\hline \hline
\textbf{w/o EPH$^{1}$} & \text{77.16$\%$}& \text{90.71$\%$}& \text{85.67$\%$}& \text{69.98$\%$}& \text{87.35$\%$}\\ \hline
\textbf{w/ EPH$^{2}$}& \text{77.77$\%$} &\text{90.85$\%$}& \text{86.14$\%$}& \text{70.20$\%$}& \text{87.08$\%$} \\ \hline
\textbf{Performance change$^{3}$}& \text{+0.61$\%$} &\text{+0.14$\%$}& \text{+0.47$\%$}& \text{+0.22$\%$}& \text{-0.27$\%$} \\ \hline
\end{tabular}
\begin{tablenotes}
\item[1] w/o EPH represents the DNN-to-be-protected, without our EPH. 
\item[2] w/ EPH indicates DNN-watermarked, with our EPH.
\item[3] The performance change of the watermarked model compared with the original model. The positive value indicates performance improvement.
\end{tablenotes}
\end{threeparttable}
\end{table}


\subsection{Comparison with State-of-the-art}
\label{subsec:comparison}
We compare our HufuNet with the state-of-the-art watermark approach~\cite{adi2018turning} mainly in the aspect of model fine-tuning. Firstly, we train Resnet18 with the same hyperparameters and the same dataset using the same pre-processing (i.e., normalization, random cropping) as in ~\cite{adi2018turning}. Then, regarding fine-tuning the model, according to~\cite{chen2019leveraging}, setting a larger initial learning rate and then properly decreasing it will effectively destruct the embedded watermark without compromising the performance of the model. So we use a larger initial learning rate of 0.05 and decrease it to 1e-7 gradually after 100 epochs by cosine annealing. To fine-tune the DNNs-watermarked using the backdoor approach \cite{adi2018turning} and our HufuNet, respectively. The two watermarks embedded into the Resnet18 model are fine-tuned using 8,000 images and verified using another 2,000 images from the CIFAR-10 testing dataset. Table \ref{tab:Contrastblackfinetuning} shows the experimental results. We find that the fine-tuning does not impact the accuracy of the watermarked models for both approaches. However, the accuracy of their backdoor based watermark~\cite{adi2018turning} drops significantly from the beginning of fine-tuning and continues decreasing as the number of epochs increases. In contrast, the accuracy of HufuNet tends to be stable, always above 92\%, resulting in 100\% ownership verification (as in Section \ref{subsec:Performance}, with $\tau_{acc} = 15\%$, above 80\% HufuNet accuracy indicates ownership verification). We also evaluate the two watermark approaches against pruning. With the pruning rate up to 60\%, we find both approaches demonstrate good robustness against pruning, with 100\% ownership verification.
%Overall, both approaches demonstrate good robustness against pruning. With the pruning percentage up to 70\%, their backdoored watermark and our HufuNet can still detect the embedded watermark with quite high confidence.Note that even if the pruning percentage is up to 90\%, HufuNet can still have the accuracy of 78.11\%. As the percentage of pruning continues increasing, our HufuNet can still claim ownership correctly, but their approach~\cite{adi2018turning} cannot.

\begin{table}
\begin{threeparttable}
\centering
\footnotesize
\caption{Comparison of Fine-tuning Performance}
\label{tab:Contrastblackfinetuning}
\begin{tabular}{m{0.7cm}
<{\centering}|m{1.24cm}
<{\centering}|m{1.1cm}
<{\centering}|m{1.24cm}
<{\centering}|m{1.0cm}
<{\centering}|m{1cm}
<{\centering}}
\hline
\multirow{2}{*}{\textbf{\makecell[c]{Epochs}}} & \multicolumn{2}{c|}{\textbf{Backdoored WM \cite{adi2018turning}}}& \multicolumn{3}{c}{\textbf{HufuNet}}\\ \cline{2-6}

\text{}&\textbf{Main task}&\textbf{\makecell[c]{SR}}&\textbf{Main task}& \textbf{Accuracy} & \textbf{SR} \\
\hline \hline
\textbf{10} & \text{91.00$\%$} &\text{42.00$\%$}& \text{92.85$\%$}&\text{92.32$\%$}&\text{100$\%$}\\ \hline
\textbf{20} & \text{91.15$\%$} &\text{37.00$\%$}& \text{92.65$\%$}&\text{92.34$\%$} &\text{100$\%$}\\ \hline
\textbf{30}& \text{91.05$\%$} &\text{35.00$\%$}& \text{92.65$\%$}&\text{92.38$\%$} &\text{100$\%$}\\ \hline
\textbf{40}& \text{90.95$\%$} &\text{29.00$\%$}& \text{92.45$\%$}&\text{92.36$\%$} &\text{100$\%$}\\ \hline
\textbf{50}& \text{90.85$\%$} &\text{25.00$\%$}& \text{92.40$\%$}&\text{92.38$\%$} &\text{100$\%$}\\ \hline
\textbf{60}& \text{90.65$\%$} &\text{26.00$\%$}& \text{92.35$\%$}&\text{92.36$\%$} &\text{100$\%$}\\ \hline
\textbf{70}& \text{90.65$\%$} &\text{26.00$\%$}& \text{92.35$\%$}&\text{92.38$\%$} &\text{100$\%$}\\ \hline
\textbf{80}& \text{90.65$\%$} &\text{26.00$\%$}& \text{92.45$\%$}&\text{92.37$\%$} &\text{100$\%$}\\ \hline
\textbf{90}& \text{90.85$\%$} &\text{25.00$\%$}& \text{92.45$\%$}&\text{92.37$\%$} &\text{100$\%$}\\ \hline
\textbf{100}& \text{90.85$\%$} &\text{25.00$\%$}& \text{92.45$\%$}&\text{92.37$\%$} &\text{100$\%$}\\ \hline
\end{tabular}
\begin{tablenotes}
\item SR indicates success rate that the watermark can verify ownership correctly.
\end{tablenotes}

\end{threeparttable}
\vspace{-4mm}
\end{table}


\ignore{\begin{table}
\begin{threeparttable}
\centering
\footnotesize
\caption{Comparison of Fine-tuning Performance}
\label{tab:Contrastblackfinetuning}
\begin{tabular}{m{0.7cm}
<{\centering}|m{1.3cm}
<{\centering}|m{1.3cm}
<{\centering}|m{1.3cm}
<{\centering}|m{1.3cm}
<{\centering}}
\hline
\multirow{2}{*}{\textbf{\makecell[c]{Epochs}}} & \multicolumn{2}{c|}{\textbf{Backdoored Watermark \cite{adi2018turning}}}& \multicolumn{2}{c}{\textbf{HufuNet}}\\ \cline{2-5}

\text{}&\textbf{Main task}&\textbf{Watermark}&\textbf{Main task}& \textbf{Watermark} \\
\hline \hline
\textbf{10} & \text{91.00$\%$} &\text{42.00$\%$}& \text{92.85$\%$}&\text{92.32$\%$}\\ \hline
\textbf{20} & \text{91.15$\%$} &\text{37.00$\%$}& \text{92.65$\%$}&\text{92.34$\%$} \\ \hline
\textbf{30}& \text{91.05$\%$} &\text{35.00$\%$}& \text{92.65$\%$}&\text{92.38$\%$} \\ \hline
\textbf{40}& \text{90.95$\%$} &\text{29.00$\%$}& \text{92.45$\%$}&\text{92.36$\%$} \\ \hline
\textbf{50}& \text{90.85$\%$} &\text{25.00$\%$}& \text{92.40$\%$}&\text{92.38$\%$} \\ \hline
\textbf{60}& \text{90.65$\%$} &\text{26.00$\%$}& \text{92.35$\%$}&\text{92.36$\%$} \\ \hline
\textbf{70}& \text{90.65$\%$} &\text{26.00$\%$}& \text{92.35$\%$}&\text{92.38$\%$} \\ \hline
\textbf{80}& \text{90.65$\%$} &\text{26.00$\%$}& \text{92.45$\%$}&\text{92.37$\%$} \\ \hline
\textbf{90}& \text{90.85$\%$} &\text{25.00$\%$}& \text{92.45$\%$}&\text{92.37$\%$} \\ \hline
\textbf{100}& \text{90.85$\%$} &\text{25.00$\%$}& \text{92.45$\%$}&\text{92.37$\%$} \\ \hline
\end{tabular}
\begin{tablenotes}
\end{tablenotes}
\end{threeparttable}
\end{table}}




\ignore{
\begin{table}
\centering
\footnotesize
\caption{Comparison of Pruning Performance}
\label{tab:contrastwithpruning}
\begin{tabular}{m{2cm}
<{\centering}|m{2cm}
<{\centering}|m{1.8cm}
<{\centering}}
\hline
\textbf{Pruning Percentage}& \textbf{Backdoored Watermark ~\cite{adi2018turning}}& \textbf{HufuNet}\\
\hline \hline
10$\%$& \text{100.00$\%$} &\text{92.34$\%$}\\ \hline
20$\%$& \text{100.00$\%$} &\text{92.33$\%$} \\ \hline
30$\%$& \text{100.00$\%$} &\text{92.42$\%$} \\ \hline
40$\%$& \text{100.00$\%$} &\text{92.28$\%$} \\ \hline
50$\%$& \text{100.00$\%$} &\text{92.18$\%$} \\ \hline
60$\%$& \text{100.00$\%$} &\text{91.62$\%$} \\ \hline
70$\%$& \text{99.00$\%$} &\text{90.69$\%$} \\ \hline
80$\%$& \text{63.00$\%$} &\text{88.99$\%$} \\ \hline
90$\%$& \text{22.00$\%$} &\text{78.11$\%$} \\ \hline
\end{tabular}
\end{table}
}


\ignore{
\begin{table}
\centering
\footnotesize
\caption{Initialization of one layer}
\label{tab:fidelity}
\begin{tabular}{m{1.5cm}
<{\centering}|m{1.1cm}
<{\centering}|m{1.1cm}
<{\centering}|m{1.1cm}
<{\centering}|m{1.1cm}
<{\centering}}
\hline

\multirow{2}{*}{\textbf{\makecell[c]{DNN}}} & \multicolumn{2}{c|}{\textbf{Resnet18}}& \multicolumn{2}{c}{\textbf{WideResnet}}\\ \cline{2-5}

\textbf{}& \textbf{Adi}& \textbf{HufuNet}& \textbf{Uchida}& \textbf{HufuNet}\\
\hline \hline
\textbf{Initialization}& \text{70.61$\%$}& \text{92.25$\%$}& \text{46.90$\%$}& \text{90.09$\%$}\\ \hline
\end{tabular}
\end{table}
}


==> arxiv2021 HufuNet/sections/Introduction.tex <==
\section{Introduction}
\label{sec:Introduction}
%-------------------------------------------------------------------------------

The rapid development of artificial intelligence and machine learning technologies in recent years has driven the broad adoption of deep neural networks (DNNs) in numerous applications such as computer vision~\cite{he2016deep,he2016identity,simonyan2014very}, natural language processing~\cite{wu2016google,collobert2011natural,xiong2016achieving}, and speech recognition~\cite{amodei2016deep,ko2015audio}. DNNs are valuable intellectual property (IP) of their owners due to the tremendous amount of expertise, effort, and computing power involved in the design, training, validating, and commercializing them. Such IP should be protected according to the IP protection law. For example, the European Patent Office has recently amended its ``Guidelines for Examination'' on how patents related to artificial intelligence and machine learning technologies should be assessed~\cite{lankinen2020patentability}. 

%In this paper, we contribute to the IP protection of white-box DNNs by proposing a novel watermarking technique, named $HufuNet$, by which owners of DNN models can claim their ownership indisputably over their models. 
Attackers with full access to the structures and parameters of DNN models may steal and possibly modify them and fraudulently claim ownership. Such IP stealing may happen in various real-world settings such as: (i) Owners outsource the training of their DNN models to third parties, (ii) Owners upload their DNN models and services to cloud service providers, and (iii) Owners license their DNN models and services to third parties. Attackers may achieve their goals via malware infection~\cite{watson2015malware,jamil2011security}, insider threats~\cite{claycomb2012insider,silowash2012common}, industrial espionage, and many other ways, leading to serious IP infringement and significant economic loss to owners.


%With the rapid development of deep learning in recent years, DNNs are widely used in computer vision[], natural language processing[] and other fields. However, training a high-performance model is a difficult task. It often requires expertise in the field of deep learning, extensive computing power, and large labeled data sets. Therefore, neural networks are often regarded as the intellectual property of owners.

%Due to deep neural networks are widely deployed and valuable, more and more attackers are targeting them. Attackers can steal models (such as, hacker external invasion or internal theft) and build illegal stolen AI services. Such theft behavior seriously violates the intellectual property and economic benefits of the owner.

%In terms of Intellectual Property (IP) protection, the European Patent Office has recently amended its 'Guidelines for Examination' about how patents related to AI and machine learning technologies should be assessed[]. Officials hope to use legal measures to protect the intellectual property of model owners. But following the current IP protection rules, the proof of model ownership requires technical means.

Watermarking, a process of hiding digital information in carrier data, has been used for media rights management~\cite{chen2001quantization,hartung1999multimedia} and software ownership protection~\cite{collberg1999software,venkatesan2001graph}. It has also been developed for the IP protection of DNNs in recent years. Most DNN watermarking techniques embed backdoors~\cite{adi2018turning,zhang2018protecting,namba2019robust,guo2018watermarking,rouhani2018deepsigns,li2019prove} into DNN models such that watermarked DNNs behave in a designed, distinguishable manner given specific inputs held by model owners as secret triggers. However, recent works \cite{chen2019leveraging,liu2018fine} show that fine-tuning~\cite{yosinski2014transferable,pittaras2017comparison} and pruning~\cite{han2015learning} can eliminate the embedded backdoors (i.e., watermarks) without significant performance loss or dramatic change of the protected models. Most existing DNN watermarking techniques are also vulnerable to fraudulent ownership claims---attackers may discover adversarial samples and use them as ``secret triggers''. It is known that adversarial samples are inherent to DNN models and can cause the models to demonstrate distinguishable behaviors ~\cite{szegedy2013intriguing,biggio2013evasion}. Attackers can claim ownership over the stolen models by querying them with adversarial samples.   

%An ideal DNN watermarking solution should achieve the following properties: (i) robustness: watermarks can still be detected by owners from stolen DNN models even if the models experienced fine-tuning, pruning and kernels cutoff/supplement (refer to Section \ref{sub:destructing}); (ii) adaptiveness: watermarks can still be detected by owners even if the model is converted to a functionality-equivalent one via structure adjustment or parameter adjustment (refer to Section \ref{sub:destructing}); (iii) stealthiness: it is difficult for attackers to learn the existence of watermark from a stolen DNN model; (iv) security: it is difficult for attackers to forge a new watermark for a stolen DNN model; (v) integrity: it is highly unlikely for DNN owners to claim ownership over innocent DNN models; and (vi) fidelity: watermark-embedding should impact little on the performance of the original DNN models.

\vspace {3pt}\noindent\textbf{Challenges in watermarking DNNs}. First, watermarks could be eliminated/undermined by attackers via fine-tuning, pruning, or kernels cutoff/supplement, by which attackers change model parameters or the number of kernels but maintain the performance of the watermarked models. The change of model parameters may effectively remove the embedded watermarks as shown in previous studies on DNN watermarking techniques~\cite{adi2018turning,uchida2017embedding,zhang2018protecting,guo2018watermarking,rouhani2018deepsigns}. Second, it is challenging to design a robust watermark without significantly sacrificing the performance of the original model. Strong robustness tends to embed a large amount of watermark information into DNN models, downgrading the watermarked models' performance to an unacceptable level. In specific applications such as autonomous driving, even 1\% of performance loss is intolerable. It is by no means trivial to find a way of embedding enough watermark information for strong robustness while keeping high fidelity of DNN models. Third, it is also challenging to prevent attackers from forging new watermarks and claim ownership fraudulently over stolen DNN models. In backdoor-based watermarking, owners of DNN models keep secret triggers as ownership proofs. However, attackers can discover adversarial samples as their triggers and confuse DNN ownership judgment effectively. Such attacks are difficult to address under the assumption that attackers understand the underlying watermarking mechanisms and explore all possible ways in forging valid watermarks to claim ownership over stolen models.
%Third, parameter level watermark is vulnerable to functionality-equivalent attack, i.e.,  converting the stolen model to a functionality-equivalent model by reordering convolution kernels or scaling neuron weights. It is challenging to always correctly retrieve the embedded watermark considering the existence of such attack.

\vspace {3pt}\noindent\textbf{HufuNet Approach}. To address these challenges, we propose $HufuNet$, a novel white-box watermarking scheme for DNN models. 
%\lpz{With our evaluation, HufuNet is highly robust to common DNN model pruning, fine-tuning and kernels cutoff/supplement, adaptive against functionality-equivalent attack, secure against watermark forgery attacks, and of high fidelity with little or no performance loss.} 
HufuNet approach can be divided into three phases: watermark generation, watermark embedding, and ownership verification. 
%\lpz{In my opinion, it is impossible for us to completely avoid mentioning such property as robustness, adaptiveness, fidelity and so on in the evaluation.} 

In the watermark generation phase, a neural network with a small number of parameters, called HufuNet, is trained to yield a high accuracy when it is tested. The set of training samples and testing samples are public references that must be used later in the ownership verification phase. 
After HufuNet is trained and tested, it is split into two pieces, with the left piece as a watermark to be embedded into a DNN model for ownership protection, and the right kept by the model owner as a secret for ownership verification.
%\lpz{(and as a benchmark, HufuNet should only trained on Fashion-MNIST, not other dataset.)}. \lpz{I also have a idea, if we can change the Fashion-MNIST name to other name(HUFU)} 
%This small neural network is also called $HufuNet$ if no confusion arises. The set of training samples (50,000 in our experiments) and the set of testing samples (10,000 in our experiments) are public references which must be used later in the ownership verification phase. The selection of these sets of samples is independent of the selection of data set for training any DNN-to-be-protected. If the DNN that is to be watermarked is a CNN model (RNN model, respectively), $HufuNet$ is designed to consist of multiple convolution layers (RNN layers, respectively) and a linear layer. 
 
In the watermark embedding phase, each convolution kernel of the left piece of HufuNet is embedded into the target DNN model's architecture that consists of a large number of parameters. The location to embed each convolution kernel is computed and selected to increase watermark forgery attack difficulty. 
%The DNN-watermarked should contain significantly more parameters than $HufuNet$ as we target at protecting large-scale DNN models rather than small-scale DNN models. After the fragments are embedded, the DNN-watermarked model is trained with its own training data. 
During the watermarked DNN model training, the parameters incorporated from HufuNet are frozen while the rest of the parameters in the model are updated. This watermark embedding process ensures that the watermarked DNN embeds the left piece of HufuNet, yet it is fully trained on its own dataset to preserve the performance on its main task. 
%The embedded $HufuNet$ information is hidden in a large DNN parameter space, which makes it difficult to be identified or removed by DNN model prowlers. 

In the ownership verification phase, the model's owner extracts the embedded watermark from a suspect DNN model at computed locations and recovers the left piece of HufuNet accordingly. Next, the owner brings out the right piece of HufuNet, merges it with the recovered left piece to form a whole HufuNet. The whole HufuNet is tested on the public set of testing samples (previously used in watermark generation). If and only if the accuracy change of the whole HufuNet (compared to the original HufuNet) is no more than a predetermined threshold, the ownership can be claimed over the suspect model. 
%Rigorous experiments show that the real owner of a DNN-watermarked can reliably verify his/her ownership even if the DNN-watermarked has been re-trained. On the other hand, it is difficult for an attacker to falsely claim ownership over a stolen DNN model. 

HufuNet is evaluated on five popular DNN models (including both CNN and RNN models) and four benchmark datasets. Experimental results show that HufuNet achieves state-of-the-art performance in the aspects as below. %of robustness, adaptiveness, stealthiness, security, integrity, and fidelity. 
In particular, after the watermark is embedded, the accuracy of these DNN models does not decline, with a 0.23\% increase on average, achieving excellent fidelity compared to their non-watermarked versions under the same training settings.
%In the worst case, the accuracy of ownership verification decreases by 2.00\%, while the accuracy of the watermarked model decreases by 42.74\%. In the best case, the accuracy of ownership verification only fluctuates by 0.07\% while the accuracy of the watermarked model is reduced by 76.52\% due to pruning. In the presence of fine-tuning attacks, each DNN model is fine-tuned for 100 epochs with a large learning rate on a benchmark dataset. 
The fine-tuning attack decreases the accuracy of the five watermarked DNNs by 1.20\% on average, but the accuracy of ownership verification decreases by only 0.36\%. When the watermarked DNN models' parameters are pruned from 10\% to 90\%, the accuracy of the watermarked DNN models may drop significantly (i.e., 61.10\% on average) to an unacceptable level. However, the accuracy of ownership verification for these pruned models drops insignificantly (i.e., 29.43\% on average). Regarding kernels cutoff attack, when 6.75\%, 2.30\%, and 4.77\% kernels are eliminated from VGG11, Resnet18, GoogLeNet respectively, we can still retrieve the remaining kernels correctly to rebuild HufuNet with watermark detection accuracy at 100\%. %\shengzhi{It looks like sometimes we use HufuNet accuracy, and sometimes use watermark detection accuracy?}
Moreover, our watermark is shown to be capable of dealing with functionality-equivalent (via structure adjustment, parameter adjustment or channel expansion) attacks without any performance downgrade. We also evaluate HufuNet against synthetic attacks, integrating fine-tuning, pruning, and functionality-equivalent attack together, and the accuracy of the retrieved HufuNet is still always above the threshold to verify the ownership as long as the adversaries would preserve the original functionality of the stolen model. The experimental results also demonstrate that statistical approaches (examining the distribution of parameter values and their gradients) cannot help learn the embedded watermark's existence. Finally, our case studies show that it is infeasible for the attacker to retrieve our HufuNet or forge a valid HufuNet for fraudulent ownership claim.
%\lpz{Finally, our case study shows the attacker can only retrieve the true HufuNet needing $2.18*10^{-4}*2^{512}$ seconds by brute force searching in our experiment setup, and the accuracy of forged HufuNet is no more than 65\%, which is far below the threshold and not enough for fraudulent ownership claim.}


%Finally, $HufuNet$ is evaluated against a variety of forging attacks. In our experiments, the highest accuracy of a forged $HufuNet$ is 59.53\%, and the average accuracy is 18.71\%. In comparison, the accuracy of ownership verification for a watermarked model is generally greater than 90\% even after significant pruning and fine-tuning. Overall, $HufuNet$ is shown highly promising for protecting large-scale DNN models in the real world.

% Yingjiu: I deleted the contribution outline below since it is not impressive. It is a weak summary of the previous part.
% Add back to have more contents.

\vspace{5pt}\noindent\textbf{Contributions}. Our main contributions are outlined below:

\vspace {2pt}\noindent$\bullet$\space\textit{New technique.} We propose a new DNN watermarking approach, which embeds a piece of the watermark into a DNN model for ownership protection and withholds the other piece for ownership verification. To the best of our knowledge, this is the first approach that splits a watermark into two pieces and combines them for ownership verification.
 
\vspace {2pt}\noindent$\bullet$\space\textit{Implementation and evaluation.} We implement our watermark HufuNet and rigorously evaluate it using both CNN and RNN models. Experimental results show that our new DNN watermarking approach can simultaneously achieve robustness, adaptiveness, stealthiness, security, integrity, and fidelity. We release our HufuNet framework to the community\footnote{https://github.com/HufuNet/HufuNet}, together with the training and testing dataset for HufuNet, hoping to contribute to the IP protection of neural network models.

%\vspace{3pt}\noindent\textbf{Roadmap}. The rest of the paper is organized as follows. Section \ref{sec:Background} introduces the background on deep neural networks, digital watermarking and watermark destructing approaches. Section \ref{sec:Motivation} presents our problem statement. Section \ref{sec:Approach} details our DNN watermarking approach. Section \ref{sec:Evaluation} evaluates our DNN watermark approach rigorously. Section \ref{sec:Related work} summarizes the related works and Section \ref{sec:Conclusion} concludes this paper. 


==> arxiv2021 HufuNet/sections/Motivation.tex <==
\section{Problem Statement}
\label{sec:Motivation}

\subsection{A Motivating Example}
With the advancement of AI techniques, neural networks are involved in various complicated tasks such as autonomous driving, speech recognition, medical diagnosis, etc. Such tasks typically rely on DNN models that are trained on a large amount of data using intensive GPU resources. For instance, the training of BERT~\cite{devlin2018bert}, a language understanding model, took 3.3 days (79.2 hours) on 4 DGX-2H servers with 64 Tesla V100 GPUs, and received \$3,751-\$12,571 bills from a cloud computing platform~\cite{strubell2019energy}. Moreover, it is estimated that training GPT-3, an autoregressive language model, would cost around \$12 million~\cite{GPT3}. Hence, protecting the IP of model owners is on demand. However, the existing backdoor-based watermarking approaches provide no sufficient protection for model owners~\cite{adi2018turning,zhang2018protecting,guo2018watermarking,rouhani2018deepsigns,namba2019robust,li2019prove}. Consider a motivating example as shown in Figure~\ref{fig:motivation}, where Alice develops a valuable DNN model $DNN_{Alice}$. Realizing the necessity of IP protection, Alice embeds several backdoor samples (i.e., triggers and their desired labels) into the model as a digital watermark $watermark_{Alice}$. Then, Alice deploys $DNN_{Alice}$ on a cloud platform in operation. 
%\shengzhi{In Figure 1, change Download to Steal.}

\begin{figure}[t]
\centering
\epsfig{figure=fig/motivation, width=0.44\textwidth} 
\caption{A Motivating Example}
\label{fig:motivation}
\vspace{-5mm}
\end{figure}

Now assume that an attacker Eve (e.g., the cloud platform provider, an insider, or a hacker) who has access to the structure and parameters of $DNN_{Alice}$ steals the model and re-commercializes it for profit. To evade Alice's detection, Eve fine-tunes and/or prunes $DNN_{Alice}$, aiming to remove Alice's watermark. To prepare for possible ownership arguments, Eve also injects a number of backdoor samples of her own choice into the stolen model as her own digital watermark $watermark_{Eve}$\footnote{Alternatively, Eve can also generate a number of adversarial examples on the stolen model as her own digital watermark $watermark_{Eve}$.}. The question is, how Alice can testify that the model $DNN_{Eve}$ is stolen from her model $DNN_{Alice}$. Alice may present her set of triggers as inputs to $DNN_{Eve}$ and observe the model's output. Even if we assume that Eve's fine-tuning and/or pruning is not effective in removing Alice's watermark, Eve can still confuse ownership verification by presenting her set of triggers or adversarial examples, thus claiming her ownership of $DNN_{Eve}$. In the worst case, the pruning and/or fine-tuning of $DNN_{Alice}$ performed by Eve removes Alice's watermark from $DNN_{Eve}$. Consequently, Eve is victorious over Alice in the dispute of ownership. 

One may argue that Alice may increase the number of embedded triggers, and use it to outperform Eve. However, such approach is not feasible. On the one hand, with the knowledge that more triggers win, Eve can simply compete with Alice by embedding more backdoors as her own watermark. On the other hand, as the number of embedded triggers increases, the accuracy of the watermarked model decreases as shown in Table~\ref{tab:numberofbackdoor} in Appendix, which limits the number of backdoors one can embed into a model. We use the backdoor injection approach described in \cite{adi2018turning} to embed different number of backdoors into VGG11 (trained on CIFAR-10), and find the accuracy drops by 1.4\% with 400 backdoor samples embedded. In addition, we obtained code from authors of \cite{adi2018turning}, applied the same setting, trained Resnet18 on CIFAR-10, repeated their experiments and got similar results as in their paper. Then we embedded a different number of backdoors into the above model, and find the accuracy drops 1.68\% with 400 backdoor samples embedded. Therefore, Alice may not want to embed too many backdoor samples as it may compromise the accuracy of the watermarked model. 




\subsection{Threat Model}
\label{subsec:threat}
We consider white-box adversaries who have full access to model structure and parameters. We assume that the adversaries, such as prowlers of neural networks, are proficient in machine learning and watermarking. To infringe on the IP of a watermarked DNN model, the adversaries may apply various machine learning techniques such as model pruning, model fine-tuning, kernels cutoff/supplement and crafting adversarial samples. Note that kernels cutoff or supplement cannot work for LSTM, since such operations will change the structure of the model, but LSTM is one piece of functional unit and its internal structure cannot be changed. Moreover, the adversaries are also capable of launching functionality-equivalent attack through structure adjustment or parameter adjustment to fail embedded watermarks. Note that such attack is only effective against CNN models for making the structure adjustment and against ReLU activation function for making the parameter adjustment. It does not work on LSTM, since it uses sigmoid as the activation function (making the parameter adjustment impossible) and the weights in LSTM must be in order (making the structure adjustment impossible). We assume that the adversaries lack necessary resources, including large-scale training datasets and sufficient computing resources, to retrain the entire or a large portion of stolen model. Finally, we also assume adversaries do not make changes beyond the functionality-equivalent and kernels cutoff attacks to the structure, which may reduce the accuracy of the stolen model to an unacceptable level.

%\lpz{According to the resources consuming and expertise level of operating DNN, we divide the attackers into three levels:}

%\lpz{Level \uppercase\expandafter{\romannumeral1}. Resource-free: There are mainly about Equivalent model attacks: Structure Equivalent and Parameter Equivalent, in this way, the attacker does not need training resources or training data, but only reorder the sequence of the convolution kernels owing to many CNN structures are equivalent upto isomorphism (Structure Equivalent); or an attacker could directly scale the weights of one neuron by a positive constant $c \textgreater 0$ and then scale the next layer by  $1/c$ and retain a functionally equivalent model (Parameter Equivalent).}

%\lpz{Level \uppercase\expandafter{\romannumeral2}. Limited-Resource: There are mainly about Fine-tuning and Pruning. In this way, the attackers only need limited-Data and Limited-Computing-Resource to fine-tune or prune to-be-protected DNN to guarantee the good performance of to-be-protected DNN.}

%\lpz{Level \uppercase\expandafter{\romannumeral3}. Sufficient-Resource and Expertise: There are mainly about generating alternative models and initializing the layers. Generating alternative models (i.e., knowledge distilling) and initializing the layers always need the attackers have a lot of training resources and training data, as well as professional knowledge to train model.} 

%\lpz{Our method is suitable for dealing with attackers of Level \uppercase\expandafter{\romannumeral1} and level \uppercase\expandafter{\romannumeral2}.}


\begin{comment}

\subsection{Design Requirements}
\label{Design_Requirements}
%We aim to achieve the following design requirements in the design of HufuNet:

\vspace {2pt}\noindent$\bullet$\space\textit{Robustness.} 
Since the adversaries are capable of model pruning, fine-tuning and kernels cutoff/supplement, it is desired that watermarks be robust against such model change operations. Even if adversaries perform such model change operations significantly on watermarked models, their owners can still detect the embedded watermarks from the changed models. 

\vspace {2pt}\noindent$\bullet$\space\textit{Adaptiveness.} Given the white-box access to model, the adversaries can launch functionality-equivalent attack via structure adjustment or parameter adjustment. Encountering this attack, the owners must ensure the embedded watermark can still be correctly retrieved to verify ownership.

\vspace {2pt}\noindent$\bullet$\space\textit{Stealthiness.}
Given a stolen DNN model, the adversaries may examine the model, either by investigating its structure and parameters, or by observing its outputs from particular inputs, to determine whether or not any watermark exists in the model. Watermark stealthiness means that it is difficult for an adversary to detect the existence of a watermark from a watermarked model. 



\vspace {2pt}\noindent$\bullet$\space\textit{Security.} Knowing watermarking approaches, the adversaries may forge their own watermarks for the DNN models they steal, and thus claim their ownership fraudulently (also called ambiguity attack~\cite{fan2019rethinking}). The security of a watermarking approach requires that it is difficult for the adversaries to forge a valid watermark for a watermarked model.

\vspace {2pt}\noindent$\bullet$\space\textit{Integrity.}
When the watermark detection approach is applied to an innocent model, the result of ownership verification should be negative as required by watermark integrity, even if the innocent model highly resembles the owner's watermarked model in various ways, e.g., trained using similar network structure or dataset. 

\vspace {2pt}\noindent$\bullet$\space\textit{Fidelity.} 
Watermark fidelity means that the performance of a watermarked model should be equivalent to the original model and that the impact of watermark embedding on the model's performance is negligible. Watermark fidelity is critical in certain DNN applications such as autonomous driving where even 1\% of performance loss is intolerable.

\end{comment}

==> arxiv2021 HufuNet/sections/Relatedwork.tex <==
\section{Related Work}
\label{sec:Related work}
%-------------------------------------------------------------------------------
%\shengzhi{Do a thorough literature review for related works, especially those about watermarking neural networks. Make sure you will not miss important related works.}
\vspace{2pt}\noindent\textbf{Watermarking neural networks.} 
%With the development of artificial intelligence technology and the improvement of computing power, DNN is now widely used in various fields. The model of DNN is an invaluable IP for its owners because DNN training requires both advanced algorithms and high-quality data sets, as well as significant computational costs. 
Uchida et al.~\cite{uchida2017embedding} proposed the idea of utilizing a parameter regularizer to embed a watermark in the parameter space of the model and retrieved it during ownership verification. However, such an approach is vulnerable to statistical analysisattack~\cite{wang2019attacks},  because the layer's parameter variance with embedded watermark is more significant than other layers without watermark. In contrast, our EPH was embedded into nearly every layer of DNN-watermarked and occupied only a small portion of its parameter space, so the variances between the layers with and without EPH are not entirely different, thus ensuring stealthiness. 

%\shengzhi{what are ghost signature and tampering attacks?} 
%\shengzhi{If you mention their approach suffer from ghost signature and tampering attacks, you need to say how our approach defeat those two attacks.}
%introduced the idea of digital of watermark, and first proposed a framework for embedding the watermark in model parameters, which is applicable to the protection of white box models. These work provide a research direction for the protection of the IP of DNN, and the latter related research all revolves around how to embed a watermark on the model. However, the premise of white box watermarking is to have access to all parameters of the target model, and DNNs are usually deployed for remote access, so the assumption is difficult to guarantee in reality.  

Recently, backdoor-based watermarking approaches have been proposed to probe black-box or grey-box neural network models that are suspects of IP infringement~\cite{adi2018turning}, \cite{zhang2018protecting}, \cite{guo2018watermarking}, \cite{rouhani2018deepsigns}. Adi et al.~\cite{adi2018turning} embedded a set of abstract images with predefined labels into DNN models to build the trigger set, which acted as digital watermarks (only known to model owners) against the suspect models. Zhang et al.~\cite{zhang2018protecting} enriched the training dataset by adding content, noise, or irrelevant class examples as triggers, and leveraged them as model watermarks. Guo et al.~\cite{guo2018watermarking} proposed a watermarking approach similar to~\cite{zhang2018protecting} that can be used on embedded devices.
%Zhang et al.~\cite{zhang2018protecting} generalized digital watermarking as a method to hide secret information in digital media to protect the ownership of those media data, and proposed a watermarking approach for model ownership verification based on image recognition, which generates a sample trigger set of backdoor watermarks by adding content, noise, or irrelevant class examples to the raw training data. 
%Rouhani et al.~\cite{rouhani2018deepsigns} watermarked both white-box and black-box models by selecting pairs of random images and random labels as watermarks (key samples) and embedding them in the probability density function of the activation set of the target layer. \shengzhi{How can this be black-box?} 
However, the backdoor watermark approaches proposed above are non-blind watermark, which either fails to defend against evasion attacks~\cite{hitaj2018have} or does not explicitly address the problem of fraudulent ownership claim. Evasion attack~\cite{hitaj2018have} evades backdoor-based watermark verification by training a powerful detector to identify key samples in the trigger set of owners, and returning a random label rather than the predefined label when it detects a key sample used as input. 

To overcome the ``non-blind'' problem, backdoor-based blind watermarking approach \cite{namba2019robust}, \cite{li2019prove} has been proposed. Namba et al.~\cite{namba2019robust} utilized the original samples in the training dataset as watermarks by changing their labels. Li et al.~\cite{li2019prove} built watermarks by integrating a specific logo into the original samples and changing their labels. Merrer et al.~\cite{le2019adversarial} proposed a zero-bit watermarking algorithm based on adversarial examples. It fine-tunes the DNN-to-be-protected, so that the produced DNN model contains certain true/false adversarial examples, which can be used as secret keys to achieving ownership verification of the DNN models. These approaches still cannot deal with the fraudulent claims of ownership, since attackers can still pretend to be owners by utilizing adversarial samples to build their own trigger set. Different from these studies, our HufuNet can achieve high robustness and security.

%\todo{Such watermarking approach is based on adversarial training, which is initially as a defense against adversarial examples and also commonly used to improve the generalization performance of neural networks~\cite{miyato2018virtual}. For this reason, this watermarking method can falsely determine models without watermark as models with a watermark~\cite{namba2019robust}}. \lpz{Those works also have a vulnerability that each model essentially has infinite such keys, therefore everyone can claim the ownership of the DNN models with any K, that is fraudulent claims of ownership. In contrast, our HufuNet can resist fraudulent claims of ownership, such as forging a HufuNet.}

\vspace{2pt}\noindent\textbf{Counterattacks against watermarking.} Uchida et al. \cite{uchida2017embedding} proposed to fine-tune or prune the DNN model to modify its parameters, thus removing the embedded watermark.
%Because of the increasing robustness of existing watermarking techniques, watermarks can be successfully validated even when the DNN model itself fails due to pruning and fine-tuning.
Wang et al.~\cite{wang2019attacks} proposed to reveal any watermark based on the change of statistical distribution of parameters of the layer where the watermark is embedded. Yang et al.~\cite{yang2019effectiveness} demonstrated that distillation-based attacks can be effective to perform watermark elimination, based on the premise that the adversaries have plenty of data to fine-tune the model. Chen et al.~\cite{chen2019leveraging} proved that the well-designed fine-tuning method can remove the watermark without compromising the function of the model with a large learning rate and unlabeled data. Hitaj et al.~\cite{hitaj2018have} proposed a method of evasion attacks against backdoor watermarks, which evade the homeowner's verification, thereby avoiding the discovery of model theft.
%Further, Chen et al.~\cite{chen2019refit} proposed a framework that removes the watermark based on fine-tuning, named REFIT, with limited data.
Although these counterattacks significantly threaten the backdoor-based watermarking, our design has better robustness against them. 

%\vspace{5pt}\noindent\textbf{Model stealing.} \shengzhi{Consider deleting the below related works, due to: 1. not quite relevant to watermarking, 2. space limitation.} Model stealing attack learns parameters~\cite{tramer2016stealing}, hyperparameters~\cite{wang2018stealing}, or architectural information~\cite{oh2019towards} of the target model, thus constructing a model with similar performance. Tramer et al.~\cite{tramer2016stealing} proposed a models stealing attack via API prediction, using non-adaptive, random queries to infer the parameters of the  target model. Orekondy et al.~\cite{Orekondy_2019_CVPR} proposed a functionality stealing attack to extract DNN attributes based on the input and output pairs of the target model，which are used to train a ``knockoff'' model. Jagielski et al.~\cite{jagielski2020high} proposed a functionally-equivalent model extraction attack by improving the learning-based attack's query efficiency. Their prediction matches the target model on all test samples without training their model weights. Model inversion~\cite{fredrikson2014privacy,fredrikson2015model,papernot2016towards,melis2019exploiting} relies on the output of some hidden input to infer certain features of it. Fredrikson et al.~\cite{fredrikson2015model} proposed a model reversal attack, which enables the recovery of images from the training dataset of the target DNN models. Melis et al.~\cite{melis2019exploiting} showed that in collaborative learning scenarios, attackers can infer sensitive attributes, e.g., gender, related to the new training dataset after the target model is updated with such dataset. Shokri et al.~\cite{shokri2017membership} first introduced membership inference attack, which aims to determine whether a given data sample is included in the training data. Salem et al.~\cite{salem2018ml} extended \cite{shokri2017membership} by relaxing its requirements, thus a more generic approach. Shokri et al. generated training data for the target model by using a shadow model to simulate the behavior of the target model. Yeom et al.~\cite{yeom2018privacy} demonstrated that under the premise that attackers can access the target model and know the average training loss of the model, overfitting may directly lead to membership inference attack.

==> arxiv2021 HufuNet/template/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> overview.tex <==
\section{Motivation}
\label{sec:Motivation}


\begin{figure}[t]
\centering
\epsfig{figure=fig/motivation.png, width=0.5\textwidth} 
\caption{\textbf{Motivation Example}}
\label{fig:motivation}
\end{figure}






\subsection{Threat Example}
\shengzhi{Motivation examples means you tell a story: a) A model owner releases their model (complicated and accurate) on github, b) adversary identifies its value and clones it, c. To avoid legal issues, adversary fine-tunes (XXX approaches) the model and adds his own watermark, d) Adversary commercializes it (make it black box as well) and gets revenue. Then you want to use the story to emphasize the need of our approach: a) black box model from adversary, so we need to probe. But since the model is complicated and adversary has done pruning, the results of probing may not be convincing. Therefore, white box verification is needed.}

As the advance of AI techniques, neural networks are involving in various complicated tasks, e.g., autonomous driving, speech recognition, remote diagnosis, etc. Such tasks usually rely on DNN models trained on a large amount of data using intensive GPU resources.
For instance, AlexNet paper[] it’s stated that “our network takes between five and six days to train on two GTX 580 3GB GPUs”. \shengzhi{Give an example of a real world complicated model trained using XXX data and XXX GPU for XXX days.} Hence, the IP of DNN models has become a vital topic in the AI community. 

Consider an example as shown in Figure\ref{fig:motivation}, Alice makes great efforts to design a complicated and accurate neural network $DNN_{Alice}$ that performs well on the main task, and embed a backdoor[] watermark to $DNN_{Alice}$. Then he publishes $DNN_{Alice}$ to models sharing platform, such as GitHub and Google Cloud AI platform []. After that, an attacker Bob thinks that $DNN_{Alice}$ is very valuable, and then stealing it. To avoid legal issues, Bob fine-tunes, prunes the model and adds his own backdoor[] watermark, generating $DNN_{Bob}$. Next, Adversary commercializes it in black box and gets revenue.  

In view of this situation, Alice needs to claim ownership of the stolen model $DNN_{Bob}$. Alice first performs black box verification on $DNN_{Bob}$, but at this time, Bob can also have some key samples constructed by AEs or from his new constructed backdoor for fraudulent claims of ownership. Moreover since the model is complicated and adversary has done pruning, the results of probing by backdoor may not be convincing. 

%\begin{figure}[t]
%\centering
%\epsfig{figure=fig/table_attacker.png, width=0.5\textwidth} 
%\caption{\textbf{Capability of Attacker}}
%\label{fig:table_attacker}
%\end{figure}

\begin{table}
\centering
\footnotesize
\caption{Capability of Watermark}
\label{tab:Capability of Attacker}
\begin{tabular}{m{2.5cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1.4cm}
<{\centering}}
\hline
\textbf{ }& \textbf{Elementary level}& \textbf{Intermediate level}& \textbf{Advanced level}\\
\hline \hline
\textbf{Fraudulent claims of ownership} & \text{\Checkmark}& \text{\Checkmark}& \text{\Checkmark}\\ \hline
\textbf{Access to White Box}& \text{-} &\text{\Checkmark}& \text{\Checkmark} \\ \hline
\textbf{Pruning and Fine-tuning}& \text{-} &\text{-}& \text{\Checkmark} \\ \hline
\textbf{Watermark Rewrite}& \text{-} &\text{-}& \text{\Checkmark} \\ \hline
\end{tabular}
\end{table}

\shengzhi{The Table needs revision. It should show how existing works and ours perform on those metrics listed in the first column.}

Moreover, we classify several levels of attackers according to the capability our attacker can have as show in Figure \ref{fig:table_attacker}.
These attackers cause great challenges to current backdoor watermarking methods. Therefore, some watermark that can play an arbitration role in ownership verification is needed, we propose $HufuNet$ which can give an arbitration result of ownership in white box. Only in this way, can Alice verify the ownership of $DNN_{Bob}$ without any controversy.


\begin{comment}
A well-trained DNN is a valuable intellectual property (IP) for its owners, officials hope to use legal measures to protect the intellectual property of model owners. And the role of the watermark is primarily to protect the IP from being infringed.

The potential security risks of the IP of DNN are watermark removing and fraudulent claims of ownership. In terms of watermark removing, previous work \textcolor{red}{[leveage] [fine-prune] [evasion]} showed that attacker $\mathbb{A}$ can increase learning rates to fine-tuning or pruning to effectively remove the black box watermark. In terms of fraudulent claims of ownership, attacker $\mathbb{A}$ can generate some AEs [X] to fraudulent claim of ownership. Both of these risks are huge challenges to black box watermark. To address the above problems, we propose a new watermark ownership framework that provides the first black box verification, and then white box ownership verification with a high robustness protection mechanism.

For the $DNN_{valid}$ of disputed ownership, we first perform a robust black box watermark verification. If the verification result is under a high degree of confidence, we will prove the ownership of $DNN_{valid}$. But in the following two cases, the black box watermarking is not enough to verify ownership, and we will utilize the more robust and trustworthy white box watermarking method. 
(1)The black box method does not prove our ownership with a high degree of confidence, but we found out it is our model through a few minor details, and then we take legal means to get the white box model of $DNN_{valid}$ for further verification. (2)Fraudulent claims of ownership. Although we can verify ownership in the black box, attackers can also generate some adversarial samples and verify them in black box. 
Similarly, we take legal means to get the white box model of $DNN_{valid}$ and performs white box verification.
\end{comment}

\begin{comment}

\subsection{Threat Model}

\shengzhi{Usually threat model is to assume the maximum capability your adversary can have. Then your approch is to deal with the worse case based on your threat model.}

The main methods of attack to eliminate the DNN watermark are pruning, fine-tuning, and watermark rewriting. Also fraudulent clams ownership attack leads to disputes over ownership. As far as these attack methods proposed, We classify several levels of attackers $\mathbb{A}$ according to the maximum capability our attacker can have as follows:

Elementary level: $\mathbb{A}$ cannot get our white box model, nor has ability of pruning, fine-tuning, watermark rewrite to our model. But he claim the ownership of our DNN rascally without any evidience.

Intermediate level:$\mathbb{A}$ does not have access to our white box model. However, they generate some AEs through queries, which in turn build trigger sets to claim ownership of the black box DNN.

Advanced level: $\mathbb{A}$ can obtain the white box model, then without pruning, fine-tuning and rewriting watermark to model. $\mathbb{A}$ didn't embed the watermark, but claimed that part of the neural network was his watermark.

Ultimate level: $\mathbb{A}$ can get access to the white box model and perform operations such as pruning and fine-tuning, further adding a similar white box secret key to claim ownership.

\end{comment}



\subsection{Design Requirements}
\shengzhi{Based on the threat model, here you can elaborate the design requirements, e.g., effectiveness, fidelity, robustness, integrity, security, etc.}

As mentioned above, we assume that attackers have a certain amount of destructive power and therefore some technical challenges need to be addressed for achieve accurate and efficient verification of watermark ownership. We conducted an in-depth analysis of the capabilities of the four levels of attackers in order to propose an excellent watermark approach.
\begin{comment}
Elementary level: Since the attacker $\mathbb{A}$ cannot get our white box model and cannot build trigger sets to verify ownership in black box, we need to design a watermark with good quality of effectiveness and integrity and security in black box verification. 

\end{comment}

Elementary level: The attacker $\mathbb{A}$ can generate some AEs to generate his trigger sample to claim ownership of our DNN, even without access to our DNN. It is a drawback to backdoor watermark to defend the attack fraudulently claim ownership. So we need to design a new watermark total different from backdoor watermark to avoid the drawback of backdoor. The new watermark shall meet the requirement as: it only can  verify the ownership of DNN which it embedded; it is difficult to fake a substitute watermark to claim ownership.

Intermediate level: Owning $\mathbb{A}$ can obtain the white box DNN and claimed that a originally part of the DNN was his watermark. In this case, we must sure our watermark with quality that watermark is undetected by attacker and it is difficult to fake a substitute watermark only by some original part of DNN and attack's local secret.


Advanced level: Due to $\mathbb{A}$ gaining the white box model, and attacking our watermark by pruning, fine-tuning, and watermark rewriting. Therefore, we need to make sure the white box watermark is of good robust to these attacks and undetected by adversary.

Moreover, a well watermark should have guaranteed a good quality that after embedding watermark, the protected DNN can not have a significant decrease in performance.

\vspace{5pt}

==> template/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

